Do Language Models Learn Semantics of Code? A Case Study in Vulnerability Detection

Recently, pretrained language models have shown state-of-the-art performance on the vulnerability detection task. These models are pretrained on a large corpus of source code, then fine-tuned on a smaller supervised vulnerability dataset. Due to the different training objectives and the performance of the models, it is interesting to consider whether the models have learned the semantics of code relevant to vulnerability detection, namely bug semantics, and if so, how the alignment to bug semantics relates to model performance. In this paper, we analyze the models using three distinct methods: interpretability tools, attention analysis, and interaction matrix analysis. We compare the models' influential feature sets with the bug semantic features which define the causes of bugs, including buggy paths and Potentially Vulnerable Statements (PVS). We find that (1) better-performing models also aligned better with PVS, (2) the models failed to align strongly to PVS, and (3) the models failed to align at all to buggy paths. Based on our analysis, we developed two annotation methods which highlight the bug semantics inside the model's inputs. We evaluated our approach on four distinct transformer models and four vulnerability datasets and found that our annotations improved the models' performance in the majority of settings - 11 out of 16, with up to 9.57 points improvement in F1 score compared to conventional fine-tuning. We further found that with our annotations, the models aligned up to 232% better to potentially vulnerable statements. Our findings indicate that it is helpful to provide the model with information of the bug semantics, that the model can attend to it, and motivate future work in learning more complex path-based bug semantics. Our code and data are available at https://figshare.com/s/4a16a528d6874aad51a0.

==> includes/save/alignment-section-old.tex <==
% We compute what considers as important for a model to make the decisions using the following three approaches, namely important set $M$. We then defined metrics, approaches and visualizations to represent the overlap between the ground truth semantics $G$ and important set $M$.
% \ben{Definitions:} Suppose we're given an AST $\astree = \langle V, E \rangle$ for each function in a dataset $D = \{ T_1, \ldots, T_{|D|} \}$.
% Using the bug queries defined in Section \ref{sec:setup}, we compute a set of features, which we denote as an ordered set $\gt \subseteq \astree$.
In this section, we compare the results of bug queries with the features which the model identified as important.
We denote the results of all bug queries as an ordered set $\gt \subseteq V$.
We then applied 3 distinct approaches to compute an \textit{un}ordered set of features which the model considers as important, denoted $\mi \subseteq V$.
We compare $\mi$ with $\gt$ with metrics unique to each approach to understand whether the model learned to distinguish bug features and associate tokens within the bug features.
% We aggregated all token-level info by the line in which it occurs.
\ben{Define ``feature''. We matched the model inputs, BPE tokens, to AST tokens by XXX method. We grouped tokens into lines using YYY method. What's the rationale?}
% We also denote cross products of $\mi$ and $\gt$ as $\miedge, \gtedge \subseteq V \times V$.
% \ben{Move this definition to the method which it's scoped - attention analysis.}
% \ben{Define ``learn semantics'' of the bug.}

We compared the models with the ground-truth semantics $G$ using the following three approaches.

\begin{itemize}
    \item Interpretation analysis: summary
    \item Attention analysis: summary
    \item Interaction attention analysis: summary
\end{itemize}

\subsection{Interpretation analysis}

\ben{MOTIVATION:}
Certain statements are important for the prediction in order to detect a bug reliably \citeme{}.
For example, a buffer overflow detector which does not consider the buffer access location cannot definitively answer whether a buffer overflow may occur; it may detect based on heuristics or spurious signals, but will always have additional uncertainty just from ignoring the fault location.

\subsubsection{Approach}

Many methods have recently been proposed to generate \textit{interpretations} of model predictions in the form of feature attribution scores.
\ben{Which to use, interpretation? Explanation? Attribution?}
We ran several interpretation tools \citeme{} on the models and compared the resulting attribution scores with the buggy feature sets.
Then, we computed Equation \ref{eq:interpretation-analysis}, where $\mi_{top(k)}$ is the set of features with the top-$k$ highest attribution scores and $\gt$ is the set of bug semantic features.
\ben{This approach does not consider combinations of tokens - only each token by itself.}
\ben{We considered several interpretation tools because the results can vary depending on the tool.}

\begin{equation}\label{eq:interpretation-analysis}
Alignment_{interpret} =
    \frac{\mi_{top(k)} \cap \gt}
    {\mi_{top(k)} \cup \gt}
\end{equation}

\subsubsection{Results}

Figure \ref{fig:interpretation-analysis-results} reports the mean $Alignment_{interpret}$ scores of all models on the D2A dataset.

\begin{figure}
\centering
\includegraphics[width=0.45\textwidth]{figures/interpretation-iou-line.pdf}
% \includegraphics[width=0.45\textwidth]{figures/interpretation-iou.pdf}
% \includegraphics[width=0.45\textwidth]{figures/interpretation-iou_switched.pdf}
% OLD PLOT
% \includegraphics[width=0.45\textwidth]{figures/interpretation-line-IoU_old-d2a_buggypaths.pdf}
\caption{Alignment of model interpretations to bug semantics; datasets are ordered by model performance (F1 score).
% \ben{Analysis: why does the alignment go down after fine-tuning? This runs counter to our claim that performance correlates with alignment. We think it is because the models \textit{learned spurious features} in order to perform highly. This would be backed up if the following is true: when the models are trained marking PVS, they perform even better and align better than the fine-tuned models.}
}
\label{fig:interpretation-analysis-results}
\end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{figures/corr-interpretation IoU.pdf}
% \caption{Correlations of $Alignment_{interpretation}$ and model performance.
% Significant results are \underline{underlined}.}
% \label{fig:interpretation-analysis-correlation}
% \end{figure}

\ben{Discuss results here.}

The models aligned more closely to PVS than to D2A buggy paths (shown in data point d2a-bp for each model).
After fine-tuning, many (XX/YY) settings have lower median alignment.
% Much lower alignment on D2A buggy paths
% 50-75\% of data at 0.0
% Sparse data above up to 1.0 alignment
% Much of the data with 0.0 alignment has 1-2 buggy lines;less skew when data filtered to 3-4 buggy lines
% Alignment low
% Highest median IoU score is 25\%
% Highest median Precision score is 50\%
% After fine-tuning, many (10/16) settings have lower median alignment (both Precision and IoU)
% This aligns with attention analysis result
% Other 4 tools give similar results; may report aggregated or mean results of all tools

\subsection{Attention analysis}

\ben{MOTIVATION:}
Bugs often require multiple operations in order to manifest.
For example, for a buffer overflow to occur, a buffer must be allocated to a certain size (event 1), then accessed outside the allocated memory region (event 2) \citeme{}.
A model that detects the bug precisely in all cases must detect both events. A detection that flags one event without the other is based on a signal that often but not always co-occurs with the bug, and thus may be a false positive.
To detect the example of a buffer overflow precisely, the model must attend to both the allocation (which determines the buffer's size) and the access location (which determines the index at which the buffer is accessed).
% \note{Difference from IoU score? Lean into the "multiple events must happen to manifest bug" angle.}

\subsubsection{Approach}

Following \cite{wanWhatTheyCapture2022,vigBERTologyMeetsBiology2021}, we analyzed the self-attention scores between tokens in relation to bug semantics.
Intuitively, a high attention score from token $i$ to token $j$ causes the model to focus more on the previous layer's encoding of token $j$ as it encodes token $i$ \cite{alammar2018illustrated}.
If the model has a high attention score between two statements in $G$, then we conclude that it has learned that these two statements are important in relation to each other.
This is evidence that the model has learned the semantics of this bug.
Note that \cite{wanWhatTheyCapture2022,vigBERTologyMeetsBiology2021} counted the number of edges within a motif, but we count the number of nodes with at least one edge within the motif (i.e. the buggy features $\gt$).
\ben{This approach does not consider order of tokens.}

To compute this, we compute Equation \ref{eq:attention-analysis}, where $\mi_{incident(\theta)}$ is the set of features joined by a high attention score (above a threshold $\theta$) and $\gt$ is the set of bug semantic features.

\begin{equation}\label{eq:attention-analysis}
Alignment_{attention} =
    \frac{\Sigma_\ds |\mi_{incidentAttention(\theta)} \cap \gt|}
    {\Sigma_\ds|\mi_{incidentAttention(\theta)}|}
\end{equation}

Informally, Equation \ref{eq:attention-analysis} measures what portion of the features joined by a high attention score are also buggy.

\subsubsection{Results}

Figure \ref{fig:attention-analysis-mean-results-d2a} reports the mean $Alignment_{attention}$ scores of all models on the D2A dataset.

\begin{figure}
\centering
\includegraphics[width=0.45\textwidth]{figures/interpretation-attention-token.pdf}
% \includegraphics[width=0.45\textwidth]{figures/interpretation-attention.pdf}
% \includegraphics[width=0.45\textwidth]{figures/interpretation-attention_old-bar.pdf}
% \ben{Don't compare paths with PVS in the same plot - they are not comparable. Since number of nodes highlighted by the model can boost the matching metric, we should use something that adjusts for the number of nodes highlighted.}
% OLD buggy paths
% \includegraphics[width=0.45\textwidth]{figures/interpretation-attention_old-d2a-bp.pdf}
\caption{Alignment of model attention to bug semantics; datasets are ordered by model performance (F1 score).}
\label{fig:attention-analysis-mean-results-d2a}
\end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{figures/corr-attention mean - compress-filter.pdf}
% \caption{Correlations of $Alignment_{attention}$ and model performance.
% Significant results are \underline{underlined}. \ben{Correction: the X axis must be the same metric.}}
% \label{fig:interpretation-analysis-correlation}
% \end{figure}

\begin{figure*}
\centering
\includegraphics[width=\textwidth,height=2in]{example-image}
\caption{Alignment of model self-attention to D2A buggy paths for some interesting models (heatmap, see \cite{wanWhatTheyCapture2022})}
\label{fig:attention-analysis-results-d2a}
\end{figure*}

\ben{Discuss results here.}

\subsection{Interaction attention analysis}

\ben{MOTIVATION:}
Many bug semantics are expressed in terms of a sequence of events \citeme{}.
For example, a null pointer dereference manifests when a pointer is assigned to NULL, then may be manipulated, then is dereferenced \citeme{}.
Each event in the sequence is necessary in order to detect the bug, and the events must happen in a certain order (e.g. dereference after assignment to NULL) for the bug to occur.
Vulnerability detection models may detect bugs by \textit{reasoning through} this chain of events.

\subsubsection{Approach}

% each cell of $\im$ assigns a probability $\im(v_i, v_j)$ to each pair in $V \times V$ which represents the probability that the node in position $j$ will be attended by the model soon after the node in position $i$.

Following \cite{paltenghiExtractingMeaningfulAttention2022}, we computed the \textit{interaction matrix} and compared it to the ordered view of bug semantics.
The \textit{interaction matrix} $\im \in V \times V$ measures, given a token in the text, the likelihood of the model moving its attention to any other token in the next layer.
Concretely, each cell of $\im$ assigns a probability $\im(v_i, v_j)$ to each pair in $V \times V$ which represents the probability that the node in position $j$ will be attended by the model soon after the node in position $i$.
The authors originally used the interaction matrix to compare the attention of large language models to human developers.
We repurposed this analysis method in order to understand the model's ``thought process'' when predicting on an example in comparison to the known bug semantics.
% Precisely, we compute Equation \ref{formula:interaction-graph} to get the interaction matrix. % Excluded because it's a long algorithm and not our work
% \ben{Explain equation}
We extended the definition to bidirectional models since we studied models with the BERT architecture, which attends to both future and past tokens, unlike GPT-like (decoder-only) models.

\ben{Why do we need the metrics, why not ``just'' use interaction matrix?}
We propose two metrics to compare the alignment of the model-important features with the interaction matrix.
\ben{What are their mutual limitations/benefits?}
Both metrics are based on the path created by joining each pair in the ordered set of nodes $\gtpath = [(\g_1, \g_2), (\g_2, \g_3), \ldots, (\g_{n-1}, \g_{n})]$ where $n = |\gt|$.
% It has $|\gtpath| = n-1$. \ben{Is it true that $\gtpath \subseteq \gtedge$?}

In the first metric, we compute the joint probability of the buggy set $\gt$ according to $\im$.
With Formula \ref{eq:joint-probability}, we decompose the joint probability into a product of the probability of each edge. This is possible because, according to the interaction matrix, each edge's probability is independent of the previously traversed path~\cite{paltenghiExtractingMeaningfulAttention2022}.
Therefore, \ben{markov property without being snooty and saying markov}.
% \item Measure probability of buggy path as $P_{\im}(\gtpath) = \prod_i^{n-1} \im((\g_i, \g_{i+1}))$.

% "Full" proof - move to appendix
% \begin{equation}
% \begin{aligned}
% \label{eq:joint-probability}
% \im(\gtpath)
% &= \im(e_1, e_2, e_3, \ldots, e_n-1) \\
% &= \im(e_1 | e_2, e_3, \ldots, e_{n-1})\im(e_2 | e_3, \ldots, e_{n-1})\\
% &\ldots \im(e_{n-1}) \\
% &\equiv \prod_i^{n-1} \im((\g_i, \g_{i+1}))
% \end{aligned}
% \end{equation}

\begin{equation}
\begin{aligned}
\label{eq:joint-probability}
\im(\gtpath)
&= \im((\g_1, \g_2), \ldots, (b_{n-1}, \g_n)) \\
&\equiv \prod_i^{n-1} \im((\g_i, \g_{i+1}))
\end{aligned}
\end{equation}

In the second metric, we induce a graph based on the most-likely edges predicted by $\im$ and measure the alignment between $\gt$ and the induced graph.
% We propose two methods to induce the graph which have complementary purposes.
% \ben{What are their mutual limitations/benefits?}
Algorithm \ref{induction-algorithm-1} builds the longest possible subsequence of $\gtpath$ using the top-$t$ most likely connections.
It also measures what portion of edges is covered by the most-likely edges in $\im$, whether or not each edge is part of a continuous path.

% \ben{Paragraphize this information}

% Metric 1: joint probability of $\gt$ according to interaction matrix
% \begin{itemize}
%     \item Define $\gtpath = [(\g_1, \g_2), (\g_2, \g_3), \ldots, (\g_{n-1}, \g_{n})]$ where $n = |\gt|$. It has $|\gtpath| = n-1$. \ben{Is it true that $\gtpath \subseteq \gtedge$?}
%     % \item given buggy path $bp = [(v_1, v_2), (v_2, v_3), \ldots, (v_{n-1}, v_{n})]$ where $v_i \in V$ and indices correspond to $\gt$ rather than entire set $V$,
%     % \item Denote element $i$ of $bp$ as $bp_i = (g_i, g_i+1)$.
%     % \item Measure probability of buggy path as $P_{\im}(\gt) = P(bp)$.
%     \item By abuse of notation, we want to compute joint probability of the buggy path, denoted $\im(\gtpath)$.
%     \item Decompose joint probability $\im(\gtpath)$ into product of probability of each edge $\prod_i^{n-1} \im((\g_i, \g_{i+1}))$. This is possible because, according to the interaction matrix, each edge's probability is independent of the previously traversed path.
%     \item Measure probability of buggy path as $P_{\im}(\gtpath) = \prod_i^{n-1} \im((\g_i, \g_{i+1}))$.
%     \item Baseline: define $B_{baseline}$ using randomly selected nodes of the same length as $B$.
%     \item Presentation: bar chart. X axis = length of path, Y axis = probability.
% \end{itemize}

% Metric 2: alignment between induced graph and $\gt$.

% \begin{itemize}
%     \item $argmax_t(x)$ returns the top-$t$ highest values in a set $x$.
% \end{itemize}

% We propose two ways to compute it.
% Both methods compute a set of nodes which is induced by combining the interaction matrix $\im$ with the bug query $\gt$.
% \begin{itemize}
%     \item Algorithm \ref{induction-algorithm-1} builds the longest possible chain out of the top-$t$ most likely connections and computes how what portion of $\gtpath$ was hit. The alignment metric is the length of the induced path.
%     \item Algorithm \ref{induction-algorithm-2} builds a (possibly disconnected) graph out of the top-$t$ most likely edges going out of the nodes in $\gtpath$. %and considers fewer disconnected subgraphs to indicate that $\im$ aligns with $\gtpath$.
%     The alignment metric is the number of components; fewer is better.
% \end{itemize}

\input{partials/induction-algorithm-1-longest-possible-chain}
\input{partials/induction-algorithm-2-most-connected-graph}

\subsubsection{Results}

We present the results of interaction analysis in Figure \ref{fig:interaction-analysis-results-d2a}.



% \ben{Presentation: bar chart. X axis = length of path, Y axis = probability.}

% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{example-image}
% \caption{Mean alignment of model self-attention to D2A buggy paths}
% \label{fig:interaction-analysis-results-d2a}
% \end{figure}


==> includes/save/improvement-intro.tex <==
Data of improvement section:
\begin{itemize}
    \item Vanilla model 
    \item Abstract PVS
    \item Abstract PVS + buggy path training, Abstract PVS testing 
    \item Ablation 1: line PVS
    \item Ablation 2: shortened PVS
\end{itemize}

In this section, we study whether a model can achieve better performance, robustness and generalization when it is better learned ground truth semantics

\subsection{Setup}
\paragraph{Robustness and Generalization Test}
\paragraph{Statement Abstraction}

In order to generalize among programs, we extracted an \textit{abstraction} of each bug query.
The abstraction is a subset of the tokens which are generally involved in the cause of a bug and not specific to a single project.
We used the following rules, including only the \underline{underlined} tokens and ignoring all other tokens:
\begin{itemize}
    \item Function calls: select only the callee name, but not operands.
    e.g. {\tt \myemph{strcpy}(a,foo(b))}.
    \item Operators: select only the operator, but not the operands.
    e.g. {\tt(a \myemph{+} b) \myemph{-} c};
    % e.g. {\tt i \myemph{++}};
    e.g. {\tt arr\myemph{[}i\myemph{++}\myemph{]}}.
\end{itemize}

We applied further filtering to buggy paths to exclude irrelevant content such as punctuation tokens and comments, and further include complete content from multi-line statements.
This included XXX\% of the D2A dataset's buggy traces..
\begin{enumerate}
    \item Extract the entire statement which contains the line/column number. This is the outermost node in the AST which contains the statement and whose type is in a list of all statement types (decl\_stmt, expression\_stmt, etc).
    \item Gather all expressions inside the statement matching certain patterns:
    \begin{itemize}
        \item call expression
        \item assignment expression
        \item operator expression
        \item array/pointer operator expression ({\tt *, ->, []})
        % \item \ben{We should look at the most common buggy traces in D2A dataset to see if we missed any of the important expressions}
        % \item \ben{After implementing, we should run through D2A dataset and observe any buggy trace lines which have no highlighted expressions. These may needed to be added to the definition.}
    \end{itemize}
    \item Extract abstraction of each expression using the above rules.
\end{enumerate}

\ben{This section must be updated with the full list of features after the experiments are completed.}

\subsection{Attend PVS}
\paragraph{Set up}
We aim to present the input to the model in a manner that directs its particular attention to potentially vulnerable statements.  To do that, we run several experiments by annotating/highlighting the potentially vulnerable statements in different ways. 

\input{figures/pvs-examples}

% Our first experiment was inserting special tokens before and after the tokens of the PVS. For example, if "malloc(n * sizeof(int))" is considered as the PVS, then the special token "\textless start\_marker\textgreater" is added before the  tokens of "malloc(n * sizeof(int))" and "\textless end\_marker\textgreater" is added after the tokens. In the second approach, we extract the leaf nodes from the AST tree of  "malloc(n * sizeof(int))" and insert special tokens before and after the tokens of each leaf node.

We found that the first two approach does not improve the performance well, while the third approach improves the performance for most of the models. Hence, we adopt the third approach to attend the PVS.


Determining which statements should be considered vulnerable statements is a challenging task. We  experimented with three different settings.

\begin{itemize}
    \item PVS V1: In this setting, we consider the following statements as PVS.
        \begin{itemize}
            \item Function call expressions that include the function name from malloc, calloc, realloc, aligned\_alloc, free, gets, scanf, strcpy, strcat; for instance, malloc(n * sizeof(int)).
            \item array/pointer operator expressions ({\tt *, ->, []} ).
            \item Operator expressions (+, -, /, *, \%).
        \end{itemize}
    \item PVS V2: This is the updated version of the setting V1. In this setting, we consider the following statements as PVS.
        \begin{itemize}
            \item Function call expressions that include the function name from malloc, calloc, realloc, kalloc, kcalloc, krealloc, valloc, vcalloc, vrealloc, free, kfree, kfree\_sized, free\_aligned\_sized, gets, puts, scanf, sprintf, strlen,strcpy, strncpy,strcat, strncat.
            \item array/pointer operator expression ({\tt *, ->, []} ).
            \item Operator expression (+, -, /, *, \%, ++, --, \/=, \%=,
            +=, -=).
        \end{itemize}

    \item PVS V3: This is the abstraction version of the setting V2.
        \begin{itemize}
            \item only the function name is marked or highlighted, but the function arguments are not. For example, in the expression malloc(n * sizeof(int)), only 'malloc' is marked or annotated.
            \item Only the array/pointer operators ({\tt *, ->, []} ) from the array/pointer operator expressions are highlighted but not the variables.
            \item Only the mathmatical operators (+, -, /, *, \%, ++, --, \/=, \%=,
            +=, -=) are highlighted from the operator expression but not the operands. 
        \end{itemize}
\end{itemize}


==> includes/save/improvement-tables.tex <==
\begin{table}[]
\centering
\caption{PVS annotation performance.}
\begin{tabular}{|l|l|r|r|r|r|}
\hline
Model     & Setting & \multicolumn{1}{l|}{D2a} & \multicolumn{1}{l|}{CXG} & \multicolumn{1}{l|}{Big-Vul} & \multicolumn{1}{l|}{Reveal} \\ \hline\hline
CodeBERT  & Vanilla & 0.6676                   & 0.569                    & 0.4065                       & 0.4269                      \\ \hline
CodeBERT  & PVS      & \textbf{0.6704}                   & 0.5346                   & 0.3814                       & \textbf{0.4366}                  \\ \hline \hline
UniXcoder & Vanilla & 0.5719                   & 0.5681                   & 0.3955                       & 0.4053                      \\ \hline
UniXcoder & PVS      & \textbf{0.6676}                   & \textbf{0.6204}                   & 0.3912                       & \textbf{0.4267}                      \\ \hline\hline
LineVul   & Vanilla & 0.6822                   & 0.5447                   & 0.8604                       & 0.4292                      \\ \hline
LineVul   & PVS      & 0.6769                   & \textbf{0.5866}                   & 0.3644                       & \textbf{0.4545}                      \\ \hline\hline
CodeT5    & Vanilla & 0.5733                   & 0.586                    & 0.402                        & 0.4056                      \\ \hline
CodeT5    & PVS      & \textbf{0.6568}                   & \textbf{0.6053}                   & \textbf{0.4096}                       & \textbf{0.4388}                      \\ \hline
\end{tabular}
\end{table}
\begin{table}[]
\begin{tabular}{|l|l|r|r|r|r|}
\hline
Model     & Setting & \multicolumn{1}{l|}{D2a}      & \multicolumn{1}{l|}{CXG}      & \multicolumn{1}{l|}{Big-Vul}  & \multicolumn{1}{l|}{Reveal}   \\ \hline
CodeBERT                          & Vanilla & 0.6676                        & 0.569                         & 0.4065                        & 0.6411                        \\ \hline
CodeBERT                          & PVS     & 0.6082                        & {\color[HTML]{FF0000} 0.5924} & 0.3835                        & {\color[HTML]{FF0000} 0.6532} \\ \hline
CodeBERT                          & PVS      & 0.5869                        & {\color[HTML]{FF0000} 0.5904} & 0.3796                        & {\color[HTML]{FF0000} 0.6601} \\ \hline
CoDeBERT                          & PVS      & 0.5784                        & 0.5678                        & 0.3727                        & 0.6354                        \\ \hline
                                  &         & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}         \\ \hline
UniXcoder                         & Vanilla & 0.5719                        & 0.5681                        & 0.3955                        & 0.6288                        \\ \hline
UniXcoder                         & V1      & {\color[HTML]{FF0000} 0.5741} & 0.5389                        & {\color[HTML]{FF0000} 0.4023} & {\color[HTML]{FF0000} 0.6434} \\ \hline
UniXcoder & V2      & {\color[HTML]{FF0000} 0.601}  & {\color[HTML]{FF0000} 0.5956} & 0.3963                        & {\color[HTML]{FF0000} 0.6556} \\ \hline
UniXcoder & V3      & 0.5                           & 0.4984                        & 0.4185                        & {\color[HTML]{FF0000} 0.6485} \\ \hline
                                  &         & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}         \\ \hline
LineVul                           & Vanilla & 0.6822                        & 0.5447                        & 0.8604                        & 0.5909                        \\ \hline
LineVul                           & V1      & 0.6579                        & {\color[HTML]{FF0000} 0.5622} & 0.3605                        & {\color[HTML]{FF0000} 0.5937} \\ \hline
LineVul   & V2      & 0.6349                        & {\color[HTML]{FF0000} 0.5878} & 0.3269                        & {\color[HTML]{FF0000} 0.6036} \\ \hline
LineVul   & V3      & 0.4625                        & 0.5489                        & 0.2769                        & {\color[HTML]{FF0000} 0.6046} \\ \hline
                                  &         & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}         \\ \hline
CodeT5                            & Vanilla & 0.5733                        & 0.586                         & 0.402                         & 0.6271                        \\ \hline
CodeT5                            & V1      & {\color[HTML]{FF0000} 0.6302} & 0.4806                        & 0.3978                        & {\color[HTML]{FF0000} 0.6474} \\ \hline
CodeT5    & V2      & 0.5263                        & 0.0467                        & 0.3917                        & 0.5406                        \\ \hline
CodeT5    & V3      & 0.632                         & 0.5637                        & {0.4052} & {0.631}  \\ \hline
\end{tabular}
\caption{PVS table with f1 score}
\end{table}
\begin{table}[]
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Model     & PVS Setting & \begin{tabular}[c]{@{}c@{}}D2A\\ Acc\end{tabular}     & \begin{tabular}[c]{@{}c@{}}CXG\\ Acc\end{tabular}     & \begin{tabular}[c]{@{}c@{}}Big-Vul\\    F1\end{tabular} & \begin{tabular}[c]{@{}c@{}}Reveal\\     F1\end{tabular} \\ \hline \hline
CodeBERT  & Vanilla     & 0.6191                                                & 0.6457                                                & 0.4065                                                  & 0.6411                                                  \\ \hline
CodeBERT  & V1          & {\color[HTML]{FF0000} 0.6275}                         & 0.634                                                 & {\color[HTML]{FF0000} 0.5507}                           & {\color[HTML]{FF0000} 0.6532}                           \\ \hline
CodeBERT  & V2          & {\color[HTML]{FF0000} 0.6278}                         & 0.6296                                                & 0.3796                                                  & {\color[HTML]{FF0000} 0.6601}                           \\ \hline
CodeBERT  & V3          & 0.6084                                                & 0.6223                                                & 0.3727                                                  & 0.6354                                                  \\ \hline \hline
UniXCoder & Vanilla     & 0.6057                                                & 0.6365                                                & 0.3955                                                  & 0.6288                                                  \\ \hline
UniXcoder & V1          & {\color[HTML]{FF0000} 0.6191} & {\color[HTML]{E06666} 0.6369} & {\color[HTML]{CC0000} 0.5535}   & {\color[HTML]{FF0000} 0.6434}   \\ \hline
UniXcoder & V2          & {\color[HTML]{FF0000} 0.6107} & 0.6303                        & 0.3963                          & {\color[HTML]{FF0000} 0.6556}   \\ \hline
UniXcoder & V3          & {\color[HTML]{FF0000} 0.6117} & 0.6321                        & {\color[HTML]{E06666} 0.4185}   & {\color[HTML]{FF0000} 0.6485}   \\ \hline \hline
LineVul   & Vanilla     & 0.5872                                                & 0.6230                                                & 0.8604                                                  & 0.5909                                                  \\ \hline
LineVul   & V1          & {\color[HTML]{FF0000} 0.6074} & 0.6127                        & 0.5334                          & {\color[HTML]{FF0000} 0.5937}   \\ \hline
LineVul   & V2          & {\color[HTML]{FF0000} 0.6258} & 0.6201                        & 0.3269                          & {\color[HTML]{FF0000} 0.6036}   \\ \hline
LineVul   & V3          & 0.6107                        & 0.6215                        & 0.2769                          & {\color[HTML]{FF0000} 0.6046}   \\ \hline \hline
CodeT5    & Vanilla     & 0.5554                                                & 0.6482                                                & 0.4020                                                  & 0.6271                                                  \\ \hline
CodeT5    & V1          & {\color[HTML]{FF0000} 0.6141} & 0.6277                        & {\color[HTML]{FF0000} 0.5613}   & {\color[HTML]{FF0000} 0.6474}   \\ \hline

CodeT5    & V2          & {\color[HTML]{FF0000} 0.5971} & 0.5421                        & 0.3917                          & 0.5406  \\ \hline
CodeT5    & V3          & 0.5987                        & 0.6329                        & {\color[HTML]{E06666} 0.4052}   & {\color[HTML]{FF0000} 0.6310}   \\ \hline
\end{tabular}
\end{table}

==> includes/save/interaction_matrix.tex <==


\subsection{Interaction attention analysis}

\ben{MOTIVATION:}
Many bug semantics are expressed in terms of a sequence of events \citeme{}.
For example, a null pointer dereference manifests when a pointer is assigned to NULL, then may be manipulated, then is dereferenced \citeme{}.
Each event in the sequence is necessary in order to detect the bug, and the events must happen in a certain order (e.g. dereference after assignment to NULL) for the bug to occur.
Vulnerability detection models may detect bugs by \textit{reasoning through} this chain of events.

\subsubsection{Approach}

% each cell of $\im$ assigns a probability $\im(v_i, v_j)$ to each pair in $V \times V$ which represents the probability that the node in position $j$ will be attended by the model soon after the node in position $i$.

Following \cite{paltenghiExtractingMeaningfulAttention2022}, we computed the \textit{interaction matrix} and compared it to the ordered view of bug semantics.
The \textit{interaction matrix} $\im \in V \times V$ measures, given a token in the text, the likelihood of the model moving its attention to any other token in the next layer.
Concretely, each cell of $\im$ assigns a probability $\im(v_i, v_j)$ to each pair in $V \times V$ which represents the probability that the node in position $j$ will be attended by the model soon after the node in position $i$.
The authors originally used the interaction matrix to compare the attention of large language models to human developers.
We repurposed this analysis method in order to understand the model's ``thought process'' when predicting on an example in comparison to the known bug semantics.
% Precisely, we compute Equation \ref{formula:interaction-graph} to get the interaction matrix. % Excluded because it's a long algorithm and not our work
% \ben{Explain equation}
We extended the definition to bidirectional models since we studied models with the BERT architecture, which attends to both future and past tokens, unlike GPT-like (decoder-only) models.

\ben{Why do we need the metrics, why not ``just'' use interaction matrix?}
We propose two metrics to compare the alignment of the model-important features with the interaction matrix.
\ben{What are their mutual limitations/benefits?}
Both metrics are based on the path created by joining each pair in the ordered set of nodes $\gtpath = [(\g_1, \g_2), (\g_2, \g_3), \ldots, (\g_{n-1}, \g_{n})]$ where $n = |\gt|$.
% It has $|\gtpath| = n-1$. \ben{Is it true that $\gtpath \subseteq \gtedge$?}

In the first metric, we compute the joint probability of the buggy set $\gt$ according to $\im$.
With Formula \ref{eq:joint-probability}, we decompose the joint probability into a product of the probability of each edge. This is possible because, according to the interaction matrix, each edge's probability is independent of the previously traversed path~\cite{paltenghiExtractingMeaningfulAttention2022}.
Therefore, \ben{markov property without being snooty and saying markov}.
% \item Measure probability of buggy path as $P_{\im}(\gtpath) = \prod_i^{n-1} \im((\g_i, \g_{i+1}))$.

% "Full" proof - move to appendix
% \begin{equation}
% \begin{aligned}
% \label{eq:joint-probability}
% \im(\gtpath)
% &= \im(e_1, e_2, e_3, \ldots, e_n-1) \\
% &= \im(e_1 | e_2, e_3, \ldots, e_{n-1})\im(e_2 | e_3, \ldots, e_{n-1})\\
% &\ldots \im(e_{n-1}) \\
% &\equiv \prod_i^{n-1} \im((\g_i, \g_{i+1}))
% \end{aligned}
% \end{equation}

\begin{equation}
\begin{aligned}
\label{eq:joint-probability}
\im(\gtpath)
&= \im((\g_1, \g_2), \ldots, (b_{n-1}, \g_n)) \\
&\equiv \prod_i^{n-1} \im((\g_i, \g_{i+1}))
\end{aligned}
\end{equation}

In the second metric, we induce a graph based on the most-likely edges predicted by $\im$ and measure the alignment between $\gt$ and the induced graph.
% We propose two methods to induce the graph which have complementary purposes.
% \ben{What are their mutual limitations/benefits?}
Algorithm \ref{induction-algorithm-1} builds the longest possible subsequence of $\gtpath$ using the top-$t$ most likely connections.
It also measures what portion of edges is covered by the most-likely edges in $\im$, whether or not each edge is part of a continuous path.

% \ben{Paragraphize this information}

% Metric 1: joint probability of $\gt$ according to interaction matrix
% \begin{itemize}
%     \item Define $\gtpath = [(\g_1, \g_2), (\g_2, \g_3), \ldots, (\g_{n-1}, \g_{n})]$ where $n = |\gt|$. It has $|\gtpath| = n-1$. \ben{Is it true that $\gtpath \subseteq \gtedge$?}
%     % \item given buggy path $bp = [(v_1, v_2), (v_2, v_3), \ldots, (v_{n-1}, v_{n})]$ where $v_i \in V$ and indices correspond to $\gt$ rather than entire set $V$,
%     % \item Denote element $i$ of $bp$ as $bp_i = (g_i, g_i+1)$.
%     % \item Measure probability of buggy path as $P_{\im}(\gt) = P(bp)$.
%     \item By abuse of notation, we want to compute joint probability of the buggy path, denoted $\im(\gtpath)$.
%     \item Decompose joint probability $\im(\gtpath)$ into product of probability of each edge $\prod_i^{n-1} \im((\g_i, \g_{i+1}))$. This is possible because, according to the interaction matrix, each edge's probability is independent of the previously traversed path.
%     \item Measure probability of buggy path as $P_{\im}(\gtpath) = \prod_i^{n-1} \im((\g_i, \g_{i+1}))$.
%     \item Baseline: define $B_{baseline}$ using randomly selected nodes of the same length as $B$.
%     \item Presentation: bar chart. X axis = length of path, Y axis = probability.
% \end{itemize}

% Metric 2: alignment between induced graph and $\gt$.

% \begin{itemize}
%     \item $argmax_t(x)$ returns the top-$t$ highest values in a set $x$.
% \end{itemize}

% We propose two ways to compute it.
% Both methods compute a set of nodes which is induced by combining the interaction matrix $\im$ with the bug query $\gt$.
% \begin{itemize}
%     \item Algorithm \ref{induction-algorithm-1} builds the longest possible chain out of the top-$t$ most likely connections and computes how what portion of $\gtpath$ was hit. The alignment metric is the length of the induced path.
%     \item Algorithm \ref{induction-algorithm-2} builds a (possibly disconnected) graph out of the top-$t$ most likely edges going out of the nodes in $\gtpath$. %and considers fewer disconnected subgraphs to indicate that $\im$ aligns with $\gtpath$.
%     The alignment metric is the number of components; fewer is better.
% \end{itemize}

\input{partials/induction-algorithm-1-longest-possible-chain}
\input{partials/induction-algorithm-2-most-connected-graph}

\subsubsection{Results}

We present the results of interaction analysis in Figure \ref{fig:interaction-analysis-results-d2a}.



% \ben{Presentation: bar chart. X axis = length of path, Y axis = probability.}

% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{example-image}
% \caption{Mean alignment of model self-attention to D2A buggy paths}
% \label{fig:interaction-analysis-results-d2a}
% \end{figure}

\begin{figure}
\centering
\includegraphics[width=0.45\textwidth]{figures/interaction_chain-probability_length-2.pdf}
\caption{Alignment of model interaction matrices to buggy paths in D2A for path length = 2.}
\label{fig:interaction-analysis-2}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.45\textwidth]{figures/interaction_chain-probability_bars.pdf}
\caption{Alignment of model interaction matrices to buggy paths in D2A decreases with longer traces.}
\label{fig:interaction-analysis-bars}
\end{figure}

==> includes/save/intro-draft-1.tex <==
\section{Introduction}
In recent years, deep learning has been extensively explored for automating software engineering tasks~\cite{allamanis2018survey,lu_codexglue_2021}.
One important yet challenging task is vulnerability detection.
Vulnerabilities cause great harm to people and corporations each year~\cite{wikipedia_databreaches_2021,ibm_cost_2021}.
Furthermore, the number of reported vulnerabilities continues to grow~\cite{cvedetails_2021}, which necessitates effective methods of detecting vulnerabilities before release.
However, vulnerabilities are difficult to detect because conventional static analyzers often have to work around imprecision, industrial-scale engineering effort, or explosive scale~\cite{distefanoScalingStaticAnalyses2019}.
To address these concerns, recent work has applied deep learning models to learn to detect bugs probabilistically based on a training dataset of known vulnerabilities.
% While deep learning has shown promise, we also see that despite F1 scores above 90, it struggles to generalize to unseen projects and bug types and handle certain features.
% While deep learning has shown promise, we also see that unlike the fields of computer vision and natural languages, vulnerability detection hardly achieved F1 score above 90, despite the effort.

Recently, pre-trained language models such as CodeBERT~\cite{feng_codebert_2020} have demonstrated state-of-the-art (SOTA) performance on several source code understanding tasks using the scheme of pre-training on a large corpus using self-supervised learning, then fine-tuning on a smaller dataset for a specific task.
% \ben{Too much} The commonly-used BERT-based models are trained with the Masked Language Modeling (MLM) objective, where the model takes as input a sequence of tokens, a fraction of the tokens are hidden, and the model is tasked with filling them in.
% Other objectives and inputs can be integrated, such as including ASTs in the input or tasking the model with identifier reconstruction~\cite{wang_codet5_2021,guo_unixcoder_2022}, but in general, 
% The model architecture and pre-training objective generally rely solely on a textual representation of code.
% Surprisingly, the models can still learn high-level patterns from the code during pre-training in order to fulfill the MLM objective.
% 
When applied to vulnerability detection, pre-trained transformer models have achieved the state-of-the-art performance of 91 F1 score~\cite{fu_linevul_2022} on a real-world vulnerability dataset~\cite{fan_msr_bigvul_2020}.
In spite of their successes, these models have critical limitations: they can focus on spurious features unrelated to bugs and can struggle to generalize to unseen projects or bug types~\cite{steenhoek2023empirical}.
These limitations prevent the model from being applied in real-world projects.
Thus, we seek to understand what the models have learned in order to understand the reasons for the models' limitations and find ways to improve them.

Recently, Wan et al. analyzed the self-attention mechanism in transformers and showed that pre-trained models of code can capture and reconstruct basic syntactic structures~\cite{wanWhatTheyCapture2022}.
This builds on work in other domains, which study the relationship of model interpretations with the structures of proteins~\cite{vigBERTologyMeetsBiology2021} and natural language~\cite{jawaharWhatDoesBERT2019}.
In another vein, Paltenghi et al.~\cite{paltenghiExtractingMeaningfulAttention2022} found that the CodeGen transformer model paid attention to similar parts of code as developers.
These and related research~\cite{rogersPrimerBERTologyWhat2020} show that the models, beyond processing sequences of tokens, learn some high-level properties of the source code.
However, it is not known whether pre-trained models of code can further capture \textit{bug semantics}, or the root causes of bugs, especially when fine-tuned for a task which requires the model to learn bug semantics.
Bug semantics involve more complex constraints and are less related to the text representation than the AST~\cite{yamaguchiModelingDiscoveringVulnerabilities2014}, so the model is less likely to learn them by default.
However, without leveraging bug semantics, we argue that the model will be unable to precisely detect certain types of bugs.
Thus it is extremely important to understand whether and how the models learn bug semantics, and if they do not, to train them to learn it.

In this paper, we define a set of features related to bug semantics and analyze how deep learning-based language models use these features, in order to answer the following questions:
% 
% To further understand why this is the case, and how to further improve the model performance, we aim to investigate:
\textit{To what extent do the models use bug root causes to make predictions?
Do models perform better when using more causal lines?}
To this end, we studied four pre-trained language models using interpretation tools, attention analysis~\cite{wanWhatTheyCapture2022}, and interaction matrix analysis~\cite{paltenghiExtractingMeaningfulAttention2022}.
We compared with two types of bug semantics: buggy paths reported by the Infer static analyzer~\cite{zheng_d2a_2021} and our own development of Potentially Vulnerable Statements (PVS), based on the framework proposed by Le et al.~\cite{le_marple_2008}.
We found that the models aligned to the PVS in some cases, but most models had less than \xxx\% alignment with potentially vulnerable statements. However, the models did not substantially align to buggy paths, having median alignment scores even below \xxx\%.
Based on this analysis, we developed two methods to annotate the PVS inside the model input. Our best annotation method improved the model F1 score in the majority of cases, by \xxx-\xxx\% and improved model alignment to PVS by \xxx-\xxx\%.

We make the following contributions:
% In this paper:
\begin{enumerate}
    \item We adapt and harmonize three distinct approaches to analyze deep learning models using interpretation tools, attention analysis, and interaction matrix analysis.
    \item Using these analysis approaches, we investigate whether deep learning models encode two types of bug semantics: Potentially Vulnerable Statements (PVS) and paths reported by the industrial-strength Infer static analyzer.
    \item We show that better-performing models aligned better to bug semantics, and while the models somewhat aligned with PVS, they failed to align strongly, and failed to align substantially to buggy paths.
    \item Therefore, we develop a novel method of annotating bug semantics and show that with this annotation, models performed better and aligned more with bug semantics.
\end{enumerate}

% \ben{Generalization has not been run yet?}

% \ben{
% Overall outline:
% \begin{itemize}
%     \item The models can align to PVS and more alignment to PVS performs better.
%     \item However the models do not align strongly to PVS.
%     \item So, we annotated the PVS and see that performance increased and hope to see that alignment increased.
%     \item Furthermore, PVS is insufficient to detect bugs. Statement-based (path-insensitive) detectors cannot detect some buggy conditions, for example, flawfinder and RATS. Path-based detectors such as Infer perform much better.
%     \item The models also do not align to buggy paths.
%     We tried to annotate them and saw some improvements, but more work is needed in this area.
%     % \item Therefore, we also annotated sources and sinks and hope to see that see that performance increased and alignment increased.
% \end{itemize}
% }

% In this paper, we defined a set of program semantics related to vulnerability detection and applied different model analysis and defined metrics to understand whether the models learned any \ben{bug} semantics, and whether it is correlated with model performance and generalization.

% Vulnerability detection is a program analysis task that requires semantics. Examples of semantics of code:
% \begin{enumerate}
%     \item execution paths
%     \item value of variables
%     \item abstraction of the top twos:
%     \begin{itemize}
%         \item value flow
%         \item sequence of statements - source, sink, sequence of buffer/integer related statements 
%         \item data flow (taint propagation)
%     \end{itemize}
% \end{enumerate}

% Pre-training: learning syntax
% \note{We may find that pretraining learned to focus on bug semantics.}

% Downstream: learning semantics 

% Compare model behavior with root causes 

% Study 1: important token analysis 
% \begin{itemize}
%     \item remove them and train again, model accuracy does not change but robustness improves
% \end{itemize}

% Study 2: important sequence of lines 

% Do we see higher attention matrix correlation when both the model and the developer have the right answers vs. when they don't?



% \begin{itemize}
%     \item attention analysis: learn source/sink relations, learn root causes?
%     \item important feature analysis: remove syntactic tokens, the model keeps the accuracy but more robust 
% \end{itemize}


% RQs understand the behaviors: learn AST, learn focus on correct regions, learn temporal semantics, learn value flow?

% Action: explain the phenomena 

% Learning semantics

% Learning semantics of vulnerability

% \ben{To measure whether the model learned bug semantics, we measured the causal alignment: alignment with root causes or likely root causes of bugs.}


==> includes/save/pvs-examples.tex <==
\begin{table}[htbp]
    \centering
    \begin{tabular}{p{3.5cm}|p{4.5cm}}
        \hline
        \textbf{Annotation Method} &  \textbf{Example}\\ \hline
         We insert comments before each PVS. &
            \makecell[l]{
            // PVS line: malloc(n * sizeof(int))  \\ malloc(n * sizeof(int)); 
            }
            
         \\\hline
        We insert special tokens before and after all the tokens of the PVS statement. & \makecell[l]{
             \textbf{PVS statements}: malloc(n * sizeof(int)) \\
             \textbf{Tokens}: 'm', 'alloc', '(', 'n', '*', 'sizeof', \\ '(', 'int', '))' \\ 
             \textbf{After annotations}: \textless start\_marker\textgreater, 'm', \\  'alloc', ......., 'int', '))',  \textless end\_marker\textgreater  \\
        } \\ \hline
              We insert special tokens before and
         after each token of the PVS statements.  &
         \makecell[l]{
             \textbf{PVS statements}: malloc(n * sizeof(int)) \\
             \textbf{Tokens}: 'm', 'alloc', '(', 'n', '*', 'sizeof', \\ '(', 'int', '))' \\ 
             \textbf{After annotations}: \textless start\_marker\textgreater, 'm', \\ \textless end\_marker\textgreater, \textless start\_marker\textgreater, 'alloc', \\ \textless end\_marker\textgreater, .......,\textless start\_marker\textgreater, '))', \\ \textless end\_marker\textgreater  \\
        }
         \\ \hline

    \end{tabular}
    \caption{Different ways of annotating the PVS statements.}
    \label{tab:pvs_annotations}
\end{table}

==> includes/save/related-work-draft-1.tex <==
\section{RELATED WORK-Shaila}
\shaila {Draft-2}

\noindent {\bf{Understanding Semantics of code}}.
One of the most difficult challenges in the emerging field of deep learning-based vulnerability detection is effectively comprehending the semantics of code. Several studies have been conducted in this domain, with a focus on both model analysis and empirical studies in software engineering (SE). LineVul \cite{fu_linevul_2022} is a notable contribution that conducts function level predictions but also allows adjustments to line level prediction after-words. LineVul utilizes CodeBERT \cite{feng_codebert_2020} for feature representation of source code with
% to capture vector representation of source code feature representation and
BERT's attention mechanism, which captures long-term dependencies in sequences, is used to find faulty lines.

On the other hand, VulBERTa \cite{hanif2022vulberta} relies on RoBERTa model and uses a custom tokenizer for internal code representation to learn the knowledge representation of code syntax and semantics. 
% On the other hand, VulBERTa \cite{hanif2022vulberta} aims to capture security vulnerabilities in source code by learning the knowledge representation of code syntax and semantics. It relies on a RoBERTa model and uses a custom tokenizer pipeline for internal code representation. 
This approach enhances source code encoding while preserving its syntactic structure by combining Byte-pair encoding mechanism with pre-defined token(AST-node type of Clang, common C/C++ API function calls and keywords, punctuations). 
% VulBERTa's effectiveness was evaluated across multiple datasets and benchmarks, establishing its competency in the field.
%The model's effectiveness was evaluated across 4 various datasets 
% (Vuldeepecker, Draper, REVEAL, and muVuldeepecker) and 2 benchmarks.
% (CodeXGLUE and D2A).

LineVD \cite{hin2022linevd} focuses more on line-level vulnerability detection, emphasizing the lines contributing to the vulnerability. Leveraging a graph neural network to generate control and data dependencies between statements, LineVD also uses CodeBERT's Byte-pair Encoding (BPE) tokenizer to encode source code tokens.

Another method, IVDetect \cite{li2021vulnerability} employs a graph-based approach. It represents the source code through a program dependence graph (PDG). To uncover critical features, an interpretable model named GNNExplainer generates a sub-graph by removing a node and examining the changes in prediction outcome.


\noindent{\bf{Role of Attention Mechanism in Transformers. }} Transformers-based models have been scrutinized for their attention mechanisms. Wan et al \cite{wanWhatTheyCapture2022} noted that the attention mechanism in pre-trained models CodeBERT and GraphCodeBERT could capture high-level structural properties of source code. They observed that self-attention weights aligned with the syntax structure, hypothesizing that tokens close to each other in the Abstract Syntax Tree (AST) should be given higher attention weights. 
Paltenghi et al \cite{paltenghiExtractingMeaningfulAttention2022} studied another  pre-trained neural model,CodeGen, focusing on the attention-weights for model's reasoning process. They proposed a post-processing method named "follow-up attention. Apart from source code, GPT-2 model was analyzed by Vig et al \cite{vig2019analyzing} , showing that  attention weights contain important syntactic information on different Part of Speech (POS) tag on natural language depending on layer depth of the transformer.

\noindent {\bf{An Empirical Comparison of Pre-Trained Models of Source Code}}
Given the high cost of obtaining annotated data for deep learning models, pre-training and fine-tuning for specific tasks have gained prominence. Wang et al \cite{wang_codet5_2021} proposed a pre-trained encoder-decoder model, CodeT5, which considers token type information and focuses on the identifiers that preserve rich code semantics. Meanwhile, Vig et al's work \cite{vigBERTologyMeetsBiology2021} on proteins, which are viewed as sequences of amino acids, illustrated how attention captures structural properties, targets binding sites, and is consistent with a classic measure of similarity between amino acids. They investigated five different Transformer protein models, and found that attention catches more higher-level representations of structure and function in deeper layer. Niu et al \cite{niu2023empirical}  conducts an emphirical study on 19 different pre-trained model with 13 SE tasks. However, they pointed out the difficulty in concluding which architecture is best for defect detection due to the complexity and variability in the models, configurations, pre-training tasks, and architectures used.


% Wan et al \cite{wanWhatTheyCapture2022} investigates the interpertability of pre-trained models (CodeBERT and GraphCodeBERT) to answer if the models can learn the syntactical structure of source code written in programming languages. Their findings indicated that attention can capture high-level structural properties of source code.

% A study on pre-trained neural model CodeGen focusing on the attention-weights for model's reasoning process was conducted by \cite{paltenghiExtractingMeaningfulAttention2022}. They introduces the concept of "follow-up attention," a novel post-processing approach derived solely from the attention signal and argue that the self-attention mechanism in transformer models reflects objective properties of the source code processed by the model.
% of the model's decision making process was conducted by 
 % Meanwhile, a study on BERT and RoBERTa \cite{htut2019attention} examines the
 % ability of attention heads to capture syntactic dependencies.

% Another pre-trained encoder-decoder model named CodeT5 was proposed by Wang et al \cite{wang_codet5_2021} that considers token type information and focuses on the identifiers that reserve rich code semantics and fuse such information into a Seq2Seq model. 
% Apart from source code, GPT-2 model was analyzed by Vig et al \cite{vig2019analyzing} , showing that  attention weights contain important syntactic information on different Part of Speech (POS) tag on natural language depending on layer depth. 



\noindent{\bf {The Role of Data Quality in Training Effective Vulnerability Detection Models}}. The quality of the training dataset is a critical factor in the effectiveness of vulnerability detection models.Chakraborty et al \cite{chakraborty_reveal_2022}  found that existing models perform poorly when applied to real-world problems due to issues like duplicate data, token based inadequate model, learning irrelevant features and imbalanced data by analyzing four Deep Learning-based Vulnerability Prediction techniques on source code. They, however, generate a real-world dataset named as REVEAL from two open-source projects, Linux Debian Kernel and Chromium where the vulnerabilities were reported by developer/user. Similarly Croft et al \cite{croft2023data} investigated the quality of different datasets for vulnerability detection, emphasizing that poor quality datasets may produce unacceptable results. They investigated 4 different dataset (Big-Vul, Devign, D2A, Juliet) with 5 attributes (Accuracy, Uniqueness, Consistency, Completeness, Currentness) on Chromium project and surprisingly  D2A dataset stands 100\% inaccurate data for this project.


\shaila{draft-2}

\noindent {\bf{Understanding Semantics of code}}.
One of the most difficult challenges in the emerging field of deep learning-based vulnerability detection is effectively comprehending the semantics of code. Several studies have been conducted in this domain, with a focus on both model analysis and empirical studies in software engineering (SE). LineVul \cite{fu_linevul_2022} is a notable contribution that conducts function level predictions but also allows adjustments to line level prediction after-words. LineVul utilizes CodeBERT \cite{feng_codebert_2020} for feature representation of source code with
% to capture vector representation of source code feature representation and
BERT's attention mechanism, which captures long-term dependencies in sequences, is used to find faulty lines.

On the other hand, VulBERTa \cite{hanif2022vulberta} relies on RoBERTa model and uses a custom tokenizer for internal code representation to learn the knowledge representation of code syntax and semantics. 
% On the other hand, VulBERTa \cite{hanif2022vulberta} aims to capture security vulnerabilities in source code by learning the knowledge representation of code syntax and semantics. It relies on a RoBERTa model and uses a custom tokenizer pipeline for internal code representation. 
This approach enhances source code encoding while preserving its syntactic structure by combining Byte-pair encoding mechanism with pre-defined token(AST-node type of Clang, common C/C++ API function calls and keywords, punctuations). 
% VulBERTa's effectiveness was evaluated across multiple datasets and benchmarks, establishing its competency in the field.
%The model's effectiveness was evaluated across 4 various datasets 
% (Vuldeepecker, Draper, REVEAL, and muVuldeepecker) and 2 benchmarks.
% (CodeXGLUE and D2A).

LineVD \cite{hin2022linevd} focuses more on line-level vulnerability detection, emphasizing the lines contributing to the vulnerability. Leveraging a graph neural network to generate control and data dependencies between statements, LineVD also uses CodeBERT's Byte-pair Encoding (BPE) tokenizer to encode source code tokens.

Another method, IVDetect \cite{li2021vulnerability} employs a graph-based approach. It represents the source code through a program dependence graph (PDG). To uncover critical features, an interpretable model named GNNExplainer generates a sub-graph by removing a node and examining the changes in prediction outcome.


\noindent{\bf{Role of Attention Mechanism in Transformers. }} Transformers-based models have been scrutinized for their attention mechanisms. Wan et al \cite{wanWhatTheyCapture2022} noted that the attention mechanism in pre-trained models CodeBERT and GraphCodeBERT could capture high-level structural properties of source code. They observed that self-attention weights aligned with the syntax structure, hypothesizing that tokens close to each other in the Abstract Syntax Tree (AST) should be given higher attention weights. 
Paltenghi et al \cite{paltenghiExtractingMeaningfulAttention2022} studied another  pre-trained neural model,CodeGen, focusing on the attention-weights for model's reasoning process. They proposed a post-processing method named "follow-up attention. Apart from source code, GPT-2 model was analyzed by Vig et al \cite{vig2019analyzing} , showing that  attention weights contain important syntactic information on different Part of Speech (POS) tag on natural language depending on layer depth of the transformer.

\noindent {\bf{An Empirical Comparison of Pre-Trained Models of Source Code}}
Given the high cost of obtaining annotated data for deep learning models, pre-training and fine-tuning for specific tasks have gained prominence. Wang et al \cite{wang_codet5_2021} proposed a pre-trained encoder-decoder model, CodeT5, which considers token type information and focuses on the identifiers that preserve rich code semantics. Meanwhile, Vig et al's work \cite{vigBERTologyMeetsBiology2021} on proteins, which are viewed as sequences of amino acids, illustrated how attention captures structural properties, targets binding sites, and is consistent with a classic measure of similarity between amino acids. They investigated five different Transformer protein models, and found that attention catches more higher-level representations of structure and function in deeper layer. Niu et al \cite{niu2023empirical}  conducts an emphirical study on 19 different pre-trained model with 13 SE tasks. However, they pointed out the difficulty in concluding which architecture is best for defect detection due to the complexity and variability in the models, configurations, pre-training tasks, and architectures used.


% Wan et al \cite{wanWhatTheyCapture2022} investigates the interpertability of pre-trained models (CodeBERT and GraphCodeBERT) to answer if the models can learn the syntactical structure of source code written in programming languages. Their findings indicated that attention can capture high-level structural properties of source code.

% A study on pre-trained neural model CodeGen focusing on the attention-weights for model's reasoning process was conducted by \cite{paltenghiExtractingMeaningfulAttention2022}. They introduces the concept of "follow-up attention," a novel post-processing approach derived solely from the attention signal and argue that the self-attention mechanism in transformer models reflects objective properties of the source code processed by the model.
% of the model's decision making process was conducted by 
 % Meanwhile, a study on BERT and RoBERTa \cite{htut2019attention} examines the
 % ability of attention heads to capture syntactic dependencies.

% Another pre-trained encoder-decoder model named CodeT5 was proposed by Wang et al \cite{wang_codet5_2021} that considers token type information and focuses on the identifiers that reserve rich code semantics and fuse such information into a Seq2Seq model. 
% Apart from source code, GPT-2 model was analyzed by Vig et al \cite{vig2019analyzing} , showing that  attention weights contain important syntactic information on different Part of Speech (POS) tag on natural language depending on layer depth. 



\noindent{\bf {The Role of Data Quality in Training Effective Vulnerability Detection Models}}. The quality of the training dataset is a critical factor in the effectiveness of vulnerability detection models. Chakraborty et al \cite{chakraborty_reveal_2022}  found that existing models perform poorly when applied to real-world problems due to issues like duplicate data, token based inadequate model, learning irrelevant features and imbalanced data by analyzing four Deep Learning-based Vulnerability Prediction techniques on source code. They, however, generate a real-world dataset named as REVEAL from two open-source projects, Linux Debian Kernel and Chromium where the vulnerabilities were reported by developer/user. Similarly Croft et al \cite{croft2023data} investigated the quality of different datasets for vulnerability detection, emphasizing that poor quality datasets may produce unacceptable results. They investigated 4 different dataset (Big-Vul, Devign, D2A, Juliet) with 5 attributes (Accuracy, Uniqueness, Consistency, Completeness, Currentness) on Chromium project and surprisingly  D2A dataset stands 100\% inaccurate data for this project.



\shaila{draft-1} 


Several remarkable studies have contributed to vulnerability prediction and model interpretation in security applications.
% ranging from traditional machine learning to advanced deep learning and neural networks.
These works focus on extracting important features for model decisions. To understand the complex attributes related to vulnerabilities, it is essential to have a reliable collection of vulnerable and non-vulnerable data. It is also required to feed qualityful data to machine learning or deep learning based models to perform better

% In terms of security application, there have been a number of remarkable researches done particularity in vulnerability prediction and explanation to validate the behavior of the models. They range from traditional machine learning methods to more advanced deep learning and neural network-based strategies for explaining the interpretations for each classification decisions made by the models. Some features definitely plays a vital role in making these predictions. 

LEMNA \cite{guo2018lemna} is a key contribution that explains the decision-making process of deep learning models, treating them as black boxes and using a mixture regression model to approximate non-linear decision boundaries and fused lasso to identify dependent features. In a similar note, 
In a similar note, a search based model-agnostic framework \cite{zou2021interpreting} interprets the predictions of deep learning models by extracting decision rules and identifying key tokens influencing predictions. This framework considers a non-linear decision boundary and the features are independent of each other while a combination of features is preferred over individual features by perturbing the examples. Notably, the framework demonstrates its effectiveness through a case study of two vulnerability detector named VulDeePecker and SySeVR.

% In a similar vein, a search-based model-agnostic framework \cite{zou2021interpreting} identifies key tokens influencing predictions and considers a non-linear decision boundary and feature interdependencies. Its high fidelity in identifying crucial features and producing understandable vulnerability rules was demonstrated through a case study with VulDeePecker and SySeVR

% One key contribution to this aspect is LEMNA \cite{guo2018lemna}, a novel framework explaining the decision-making process of deep learning models. It treats deep learning models as a black box, applying a mixture regression model for approximate non-linear decision boundaries and fused lasso to identify dependent features. However, LEMNA's focus is primarily on model interpretability rather than vulnerability prediction. A search-based model-agnostic framework \cite{zou2021interpreting}
% for interpreting the predictions of deep learning models extracts decision rules by identifying key tokens that significantly influence the predictions. This framework considers a non-linear decision boundary and the features are independent of each other while a combination of features are preferred over individual features by perturbing the examples. It also showcases the framework's effectiveness through a case study of  VulDeePecker and SySeVR, demonstrating its high fidelity in identifying important features and producing comprehensible vulnerability rules.


The DeepVD model \cite{wang2023deepvd}, a graph-based neural network, enhances class-separation features between vulnerable and benign code using three types of features at varying abstraction levels. An empirical study by Steenhoek et al.\cite{steenhoek2023empirical} further investigates the variability among model outputs and the importance of key features in predictions. 
% An empirical study conducted by Steenhoek et al.\cite{steenhoek2023empirical}  investigates the key features for predictions and reveals the variability among model outputs.
Another notable work is IVDetect \cite{li2021vulnerability} which also adopts a graph-based neural network but focuses on predicting vulnerabilities at the function level and provides interpretations in vulnerable statements. However, this method has been noted for its lack of accuracy and coarse granularity. 
% IVDetect \cite{li2021vulnerability}, another graph-based neural network, predicts vulnerabilities at the function level but is known for its lack of accuracy and coarse granularity. 
Recent Transformer-based models like LineVul \cite{fu_linevul_2022} have addressed these limitations, offers a better understanding of contextual relationships in data
% leveraging the ability to understand contextual relationships in data more accurately and
operating at a more resource-efficient line-level granularity. However, the complexity of Transformer-based models often leads to low interpretability.

% Recent advancements in ML/DL, particularly with Transformer-based models, have started to show even more significant accuracy , and this led to the development of LineVul \cite{fu_linevul_2022}. This Transformer-based model was proposed to handle the limitations of the state-of-the-art IVDetect approach. While other granularity levels like file,function and method level tend to have more resource-intensive and less accurate compared to the line-level prediction,  LineVul has the ability to understand contextual relationships in data more accurately. 


Therefore, several studies have aimed to understand how attention mechanisms work. For example, Wan et al. \cite{wang_codet5_2021} investigates self-attention weights in relation to code syntax, revealing that neighboring tokens 
% close in the Abstract Syntax Tree (AST) 
receive higher attention. Thus capturing high-level structural properties of source code. Abnar and Zuidema \cite{abnar2020quantifying} on self-attention mechanism propose post-hoc methods, "attention rollout" and "attention flow," to analyze the flow of information through Transformer models and provides an approximation of the relative importance of input tokens. Paltenghi et al. \cite{paltenghiExtractingMeaningfulAttention2022} propose a new follow-up attention mechanism and introduces visual attention, a static view indicating critical input parts and an interaction matrix, a dynamic view suggesting the subsequent points of interest in code based on the current position for code exploration. Meanwhile, a study on BERT and RoBERTa \cite{htut2019attention} examines the ability of attention heads to capture syntactic dependencies.
% and finds that while some heads track particular types of dependencies, none are particularly good at comprehensive parsing.


Additionally, Tutek and Snajder \cite{tutek2020staying} indicate that the lack of a word-level objective could cause attention weights to fail as faithful interpretive tools. They propose regularization methods to enhance the input-hidden state relationship. In this context, Vig Belinkov \cite{vig2019analyzing} analyzes the structure of attention in the GPT-2 small pre-trained model, finding that attention targets different parts of speech (POS) at different layer depths.
% Specifically, the model's attention aligns most strongly with dependency relations in the middle layers, while the deepest layers effectively capture the most distant relationships.

In recent years,  transformer-based models such as \cite{ahmad2021unified}, \cite{fu_linevul_2022}, \cite{feng_codebert_2020}, \cite{guo_unixcoder_2022}, \cite{guo_graphcodebert_2020} have been developed, specifically targeting vulnerability detection. However, these models have not been designed to give particular attention to specific tokens. In contrast, some research has guided the model to focus on certain tokens, primarily for program repair tasks. For instance, Modit \cite{chakraborty2021multimodal} and SequenceR \cite{SequenceR} have wrapped the buggy code with special tokens, namely $<start>, <end>$, to guide the model about the buggy lines.

Inspired by these approaches, we designed an approach to guide the model about the Potential Vulnerability Statements (PVS), enabling the model to provide special focus on these statements as well considering buggy paths. This advancement opens up new possibilities for enhanced accuracy and specificity in vulnerability detection, shedding light on the importance of target-oriented focus in machine learning models.

==> includes/save/related-work-draft-3.tex <==
\section{RELATED WORK-Shaila}


\shaila {Draft-3}

% \noindent{\bf{Learning based model dependency and semantics of code}}
Several remarkable studies have contributed to vulnerability
prediction and model interpretation in security applications. These works focus on extracting important features and their impacts on model's decision making process at different granularity level and different code representation methods such as lexical token \cite{russell2018automated}, program dependent path/value flow path \cite{cheng2022path}, program slice (\cite{li2018vuldeepecker, li2021vuldeelocator,hanif2022vulberta, li2021sysevr}), program dependency graph (PDG) \cite{li2021vulnerability}, code property graph (CPG) (\cite{zhou_devign_2019, chakraborty_reveal_2022}).
% , are commonly used to capture the important features. 

Russell et al. \cite{russell2018automated} generates important tokens from raw source code through a custom lexer discarding code comments . Standard C/C++ keywords, operators, separators are considered crucial tokens. VulDeePecker\cite{li2018vuldeepecker}, VulDeeLocator\cite{li2021vuldeelocator}  and VulDeBERTa\cite{hanif2022vulberta} generates program slices as  by extracting library/API and function calls of the source code where VulDeBERTa\cite{hanif2022vulberta} can even handle nested system calls. 
 % replacing user-defined functions and variables with abstract symbolic representations.
 SySeVR \cite{li2021sysevr} creates program slices as syntax characteristics (function call /pointer usage), semantic information (lines of code related to syntax character) using program dependency graph. ContraFlow \cite{cheng2022path} solely works on value flow paths extracted from unlabeled source code through path-sensitive code embedding.
% Devign\cite{zhou_devign_2019} and Reveal\cite{chakraborty_reveal_2022} uses code property graph (CFG) to extract the features. 
IVDetect \cite{li2021vulnerability} uses program dependency graph
and an interpretable model named GNNExplainer to generates a sub-graph by removing a node and examining the changes in prediction outcome as a feature extraction method. 

VulDeeLocator\cite{li2021vuldeelocator} provide more attention to the program slice they generate to train the model for better performance whereas
IVDetect\cite{li2021vulnerability} implemented a post processing to improve the model performance with attention .



There are also studies that explored interpretability tools, such as attention mechanisms, to understand the attention impacts in a model's decision-making process.

LineVul methods \cite{fu_linevul_2022}
uses self-attention mechanism to generate a score for each token. Tokens are intregrated to lines and those associated scores are summarized to generate line level score. Highest scores reflect the most vulnerable line. Research by Wan et al. \cite{wanWhatTheyCapture2022}, Paltenghi et al. \cite{paltenghiExtractingMeaningfulAttention2022}, and Steenhoek et al.\cite{steenhoek2023empirical} analyze the self-attention weights and their relations to the syntax of code. CodeT5\cite{wang_codet5_2021} considers providing high attention to token type information and focuses on the identifiers that preserve rich code semantics whereas \cite{paltenghiExtractingMeaningfulAttention2022} proposes a post-processing follow-up attention method for model's decision making process. 
% Apart from source code, GPT-2 model was analyzed by Vig et al \cite{vig2019analyzing} , showing that  attention weights contain important syntactic information on different Part of Speech (POS) tag on natural language depending on layer depth of the transformer. 
Vig et al. \cite{vigBERTologyMeetsBiology2021} investigates on five different Transformer protein models and found that attention catches more higher-level representations of structure and function in deeper layer.

Although, there are different transformer-based models \cite{ahmad2021unified, fu_linevul_2022, feng_codebert_2020, guo_unixcoder_2022, guo_graphcodebert_2020} for vulnerability detection process, they are not designed to give particular attention to specific tokens not even considering the buggy path. However, some research has guided the model to focus on certain tokens, primarily for program repair tasks. For instance, Modit \cite{chakraborty2021multimodal} and SequenceR \cite{SequenceR} have wrapped the buggy code with special tokens, namely $<start>, <end>$, to guide the model about the buggy lines. Therefore, we designed an approach to guide the model about the Potential Vulnerability Statements (PVS) as well as buggy paths, enabling the model to provide special focus on these statements.



==> old/action.tex <==
%\section{Results: Explaining the Models}
{\bf RQ3.1} why model X cannot perform well on the dataset A, but perform well on the dataset B? - global explanation

{\bf RQ3.2} what makes examples difficult?
using v information to compute the difficulty score and then observe if their root cause lines and tool behavior overlap? 

{\bf RQ3.21} Why this example failed to be predicted? 
Is it because  the important features do not match root cause lines?


{\bf RQ3.22} What spurious features caused misclassfications? Are there similarlity across models?

\wei{lead: Ben}

Study both in-distribution and out-distribution misclassified examples


Example inspection: For all the studies, except some summary statistics, we also should find some interesting examples
\begin{itemize}
\item Not much overlap with casual, but predict correct
\item Not much overlap with noncausal, but predict incorrect
\end{itemize}

Hypothese for the above two: Model is not able to use root cause lines, but spurious features, but surious features are not available in the OOD dataset

{\bf RQ3.3} apply off-the-shelf, generalization techniques, and explain why it can work

Hypothese: more align with the root causes?


%\section{Results: Improving the Models}




==> old/approach.tex <==
\section{Approaches}

\subsection{Attention analysis}
Step 1: design semantic queries. \textbf{[Seq]} queries are sequences of statements in the buggy path; \textbf{[Stmt]} queries are individual statements.
\begin{enumerate}
    \item paths from static analysis tools (D2A) {\bf [Seq]}
    \item pvs (potentially vulnerable statement): buffer access, integer arithmetic, pointer dereference, division, free {\bf [Stmt]} 
    \item special values, NULL pointers {\bf [Stmt]}
    \item source, sink (resource leaks), source sink pairs {\bf [pair]}
    \item value flow between the source and sink {\bf [pair]}
    \item pvs def and data dependencies - length one (buffer overflow, integer overflow, divide by zero) {\bf [Seq]}
    \item pvs control dependency, null pointer check, permission checks {\bf [Seq]}
    \item buggy commit messages (MSR)
\end{enumerate}

Semantics - provided by users via bug specification or program control, data flow information; 
\begin{itemize}
\item Constants: 0, NULL
\item Sensitive operations:pvs
\item Data types
\item Entry point
\item Control flow: resource leak, if check
\item Value flow
\end{itemize}

Can model (1) identify these elements and (2) then compose them?


Step 2: apply existing tools to perform semantic queries to attention
\begin{itemize}
    \item yes/no, or
    \item quantitative measure 
\end{itemize}

\note{The model should retain some policies learned during pretraining, such as attending to syntax. In other words, not all heads of the model should align with bug semantics. We need to account for this while designing our metrics.}

\discussion{Suggest adding models for other tasks beyond vulnerability detection.
What would the general semantics be for the first bullet point, since we will not likely have a buggy condition inside the code?
\begin{itemize}
    \item Maybe it can be cfg, dfg, and such?
    \item value flow, "values"
    \item API protocols, dependencies, temporal sequences of statements
    \item type information
\end{itemize}
}

Alignment metrics:
{\color{blue} Wei \% of high attention edges in the buggy paths}
\begin{enumerate}
    \item How to analze \textbf{[Seq]} queries?
    These queries return a buggy path $bp = [ bp_1 , \ldots, bp_n ]$ where each element $bp_i$ is a program statement. \note{For discussion: current methods only analyze attention and do not observe word embeddings, which may contain valuable indications of the model's captured information. Should we add experiments which focus on word embedding, maybe scoping out some attention-based methods to make room?}
    \begin{enumerate}
        \item \textbf{Alignment metric 1:} Attention analysis from ICSE22 paper. What proportion of token pairs which have high attention scores are in the buggy path?
        Precisely, compute Equation \ref{attention-alignment-1} given:
        \begin{itemize}
            \item a corpus of code sequences $C$ where each example is a sequence of tokens $c_i = [w_1, \ldots, w_m]$,
            \item attention matrix $\alpha \in \mathbb{R}^{m \times m}$,
            \item indicator function $f(w_i, w_j)$ which returns 1 if $w_i$ and $w_j$ are both in $bp$ and 0 otherwise,
            \item attention threshold $\theta$,
% \newcommand{\sumovertokenpairs}{$\Sigma_{c \in C} \Sigma_{i = 1}^{|c|} \Sigma_{j = 1}^{|c|}$}
% \newcommand{\indicator}{$\mathbbm{1}_{\alpha_{i,j}(c)>\theta}$}
\begin{equation}\label{attention-alignment-1}
    p_{\alpha}(f) = \frac
{\sum_{c \in C} \sum_{i = 1}^{|c|} \sum_{j = 1}^{|c|} \mathbbm{1}_{\alpha_{i,j}(c)>\theta} \cdot f(w_i, w_j)}
{\sum_{c \in C} \sum_{i = 1}^{|c|} \sum_{j = 1}^{|c|} \mathbbm{1}_{\alpha_{i,j}(c)>\theta}}
\end{equation}
        \item Intuitively, we measure, only for the tokens which are above a threshold $\theta$, what proportion are also inside the buggy path.
        If $\mathbbm{1}_{\alpha_{i,j}(c)>\theta}$ is 1 for many tokens in $bp$, then $p_{\alpha}(f)$ will be close to 1.
        \item \discussion{We will flip it to measure ``What proportion of token pairs which are in the buggy path have high attention scores?''}
        \end{itemize}

        \item We can use interaction graphs from ICLR23 paper, in two ways.
        \discussion{With this metric, matching longer paths is harder. Consider modifications:
        \begin{itemize}
            \item Filter factors using a threshold
            \item Weight each factor (what are the weights?)
            \item Only factor in the top-k probabilities out of the chain
            \item Display each length of chain separately (length = 1 prob = xxx, length = 2 prob = yyy). Only works for small set of probabilities - most examples have 1-4 steps in the buggy path
        \end{itemize}}
        \begin{enumerate}
            \item \textbf{Alignment metric 2:} Measure conditional probability of the buggy path.
            % Given a buggy path $bp = [ bp_1 , \ldots, bp_{|bp|} ]$, this is measured as $P(bp) = P(bp_1) \cdot P(bp_2 | bp_1) \cdot P(bp_3 | bp_1, bp_2) \cdot \ldots \cdot P(bp_{|bp|} | )$
            Given $bp$, this is measured using Equation \ref{attention-alignment-2} according to the chain rule\footnote{\url{http://www.cse.unsw.edu.au/~cs9417ml/Bayes/Pages/Joint_Probability.html}}.
\begin{align}\label{attention-alignment-2}
    &P(bp) = P(bp_n,bp_{n-1},\ldots,bp_1) \nonumber
    \\ &= P(bp_1) P(bp_2|bp_1) P(bp_3|bp_2,bp_1) \ldots P(bp_n|bp_{n-1},\ldots,bp_1)
\end{align}
            \discussion{
                \begin{itemize}
                    \item How to get $P(bp_i | bp_{i-1},..,bp_{1})$?
                    \item We only have $$P(bp_i|bp_{i-1}), P(bp_{i-1} | bp_{i-2}),... P(bp_2 | bp_1)$$.
                    \item Each of the $P(bp_i | bp_{i-1})$ is independent. Is not it?
                    \item If they are independent, then we can use 
                    $$P(bp) = P(bp_i|bp_{i-1})* P(bp_{i-1} | bp_{i-2})*... *P(bp_2 | bp_1)$$
                \end{itemize}
            }
            
            \item \textbf{Alignment metric 3:} Measure alignment between "most-likely graph" induced from the interaction graph $S$ and buggy path $bp$.
            
            \discussion{\begin{itemize}
                \item Consider backwards traversal of buggy path.
                \item Consider using threshold instead of selecting top-k; include all interactions where probability > xxx.
            \end{itemize}}
            
            \begin{itemize}
                \item The interaction matrix is a matrix of real numbers $S \in \mathbb{R}^{m \times m}$ where $m$ is the number of code tokens and each row $S_i$ is a vector of probabilities $[S_{i,1}, \ldots, S_{i,m}]$ where $S_{i,j}$ is the probability of attention moving from token $i$ to token $j$.
                \item $argmax_t(x)$ returns the indices of the top-t highest values in a set $x$.
            \end{itemize}
            We propose two ways to compute it.
            \begin{itemize}
                \item Algorithm \ref{temporal-attention-1} builds the longest possible chain out of the top-$t$ most likely connections and compares its size to $bp$. The alignment metric is the length of the chain.
                \item Algorithm \ref{temporal-attention-2} builds a (possibly disconnected) graph out of the top-$t$ most likely connections and considers fewer disconnected subgraphs to indicate that $S$ aligns with $bp$. The alignment metric is the number of components; lower is better.
            \end{itemize}



    \item How to analyze \textbf{[Stmt]} queries?
        \begin{enumerate}
            \item \textbf{Interpretability/word importance tools?} What about the results from ``Attention is not Explanation''?
            \item \note{All \textbf{Seq} queries can be reduced to \textbf{Stmt} queries by looking at the fault location + other notable locations.}
        \end{enumerate}
        \end{enumerate}
    \end{enumerate}
\end{enumerate}

Step 3: attend the model to see performance improvement

\begin{itemize}
    \item attend the above semantic features and see how the models performance and generation changes 
    \begin{itemize}
        \item Graphcodebert did similar -- modify attention weights according to dataflow relationships and saw some improvements
    \end{itemize}
    \item or add annotations to data to increase importance of semantic features. "On Multi-Modal Learning of Editing Source Code" \url{http://arxiv.org/abs/2108.06645}
\end{itemize}

Our findings are model may cover some root causes 

\subsection{Comparing important features with causal lines}

Agreement between neral model and static analysis tools/commit messages 

\note{Previous experiments on this point considered only the line-level granularity. Since attention analysis will consider token/statement-level granularity, we may consider revising these experiments to match the same granularity.}

\subsection{Perturbation study}

spurious features: like DEBUGGING

==> old/old.tex <==
\section{Old version}
how do we construct training dataset that disable the learning of spurious features? 

How to construct a benchmark to test generalization of the models? Can that be general across the models?

\begin{itemize}
\item Does the model learn selecting features based on the (program) context?
\item Does the model learn co-features and feature dependencies to make the prediction?
\end{itemize}

{\bf RQ2} are any pairs of features always highlighted together? are any sequences of features always highlighted together?

\wei{Lead: Rasel and Sanjida}

{\bf RQ3} features are highlighted context sensitive? under certain context?

\wei{Lead: Rasel}

Similarity around highlighted features (how to define context: neibouring tokens, lines, important tokens)



==> old/rq.tex <==
\section{research questions}

Two approaches:

\subsection{Analyzing important features}

(1) What are the important features? normalize them based on their frequencies 

{\bf RQ1} which features are important? Their selection is context sensitive

\wei{Lead: Rasel}

for different labels: all, prediction correct, prediction incorrect

different vultypes

training and test sets 

agreement across different random seeds and models

top 10, 30, 50

(2) Understand how the models might use important features to make predictions? approach ---- check the sequences of lines the model focuses on

Pretrain and downstream model?

Can we query the semantics?

\subsection{Analyzing the intersection of important features and casual lines}

Preparation: 
\begin{itemize}
\item Features: Token, node, lines 
\item VulType: different types, and overall
\item Dataset: all, correct, incorrect, test, train, in-distribution, out-of-distribution
\item Root cause lines: static analysis, commit diffs 
\end{itemize}

{\bf RQ2} Are those features spurious? What are the spurious features the models rely on the current model? a study of overlapping with root cause lines and transformation studies

\wei{Lead: Ben}

(1) Overlap studyhttps://www.overleaf.com/project/63c07aa8d17288aff4425c4b

(2) Transformation study
\begin{itemize}
\item Use the trained model to test on causal lines only
\item Use the trained model to test on non-causal lines only
\item Use the trained model to test on important (top x) and also causal lines
\item Use the trained model to test on important lines (top x) only=> do the models only rely on important lines?
\item If we train the model using only causal lines and non-vulnerable programs, can be improve the accuacy (would this be useful to help the model focus on the right lines?)
\end{itemize}

Bag of local features - generate programs that do not make sense, but contain spurious features, still can predict correctly or not?

{\bf Conclusions} models are not casual (using all the root lines to make decisions), it uses some causal lines as well as spurious features to make the decisions

{\bf RQ3} Are the models performing better and generalize better when causal lines are used?

the models perform better when using causal lines to predict even the example/project has not been seen before?

\wei{lead: Ben}
Approach: 
\begin{itemize}
\item Compute the alignment of causal lines and important  between correct vs incorrect dataset
\item between training vs testing dataset
\item between in-distribution vs out-of-distribution dataset
\item Construct the best case dataset (test dataset) and worst case dataset regarding the alignment (using our metrics), then show there are big differences in terms of F1, accuracy
\end{itemize}


Others: 
\begin{itemize}
\item Any repetition patterns in the causal line that we can pick up?
\end{itemize}

Maybe we can improve the model by adding an incentive for attending to causal lines

==> partials/discussion/metrics-01.tex <==
\ben{Below are the notes from our discussion}

Comparison granularity: line or tokens as elements in the set (Line-level integration : max, sum or average)

Ground truth: set; Output: set (Select “top” elements: top-k, k is the number of truth)

Set elements: 
\begin{itemize}
    \item PVS
    \item Buggy paths
\end{itemize}

Ground-truth data
\begin{itemize}
    \item D2A buggy path
    \item PVS: char *x = malloc(1000);
    \begin{itemize}
        \item Line-level PVS : char *x = malloc(1000);
        \item Token-level PVS : malloc(1000)
        \item Abstract token-level PVS : malloc
    \end{itemize}
\end{itemize}

Set comparison:
\begin{itemize}
    \item Metrics:
    \begin{itemize}
        \item IoU
        \item percentile (how many attended lines are in the buggy paths, what portion of buggy lines are in X\% of importance)
        \item precision (what portion of attended lines hit the ground truth)
    \end{itemize}
    \item Aggregate scores in each line: mean/max/sum
    \item Select “top” elements: Threshold/top-k, what is k
\end{itemize}

Baselines:
\begin{itemize}
    \item Compare pretrained model with fine-tuned model: how does the fine-tuned dataset help improve the alignment?
\end{itemize}

==> partials/discussion/metrics-02.tex <==
\ben{DISCUSSION: The below bullet list summarizes the 3 alignment metrics in notation which is as unified as possible. It will be moved into the appropriate sections after discussion.}

\ben{Overall: BPE $\rightarrow$ token $\rightarrow$ line, How do we handle D2A buggy paths}

Metrics:
\begin{enumerate}
    \item Interpretability tools:
    \begin{itemize}
        \item Define $\mi$ as the top-$k$ nodes sorted by attribution score.
        \item Define $\gt$ as the result of the bug query.
        \item The metric is IoU for each program: $\frac{\mi \cap \gt}{\mi \cup \gt}$
        \item \ben{Aggregate by line or token? Average attributions over line vs. AST token vs. BPE token.}
    \end{itemize}
    % \item A ``feature'' is a node $v \in V$.
    \item Attention analysis (edge-wise):
    \begin{itemize}
        \item Notes from discussion:
        \begin{itemize}
            \item \ben{Currently defined at Token level. Should we swtich to line level? Aggregate all tokens in the line with mean/max/sum}
            \item \ben{Currently defined as bidirectional - even if edge $x \rightarrow y \in \miedge$, it's not necessarily true that $x \leftarrow y \in \miedge$. Consider changing so that we include both directions of any edge where at least one direction is above the threshold. Note that with bidirectional, we have 3 states: not matched, partially matched (one direction), and fully matched (both direction
            s). After changing, we have only both unmatched or both matched. If we think this will increase alignment, then we are positing that there are many partially matched edges and not many fully matched edges, therefore the alignment is being considered as very low.}
            \item \ben{Consider using threshold attention-score above $\theta$ OR top-$k$ where $k = |\gt|$.}
        \end{itemize}
        \item Define $\miedge$ as the set of edges with attention score above a threshold $\theta$.
        \item Define $\gt$ as the result of the bug query.
        \item Define $\gtedge$ as the cross product of $\gt$.
        \item The metric is the portion of $\miedge$ which is also in $\gtedge$.
        Formula for each attention head: $\frac{\Sigma_\ds |\miedge \cap \gtedge|}{\Sigma_\ds|\miedge|}$ where $D$ is the entire dataset.
        % There are a few ways to calculate it.
        % \begin{itemize}
        %     \item for each program, for each head: $\frac{|\miedge \cup \gtedge|}{|\miedge|}$.
        %     \item for entire dataset, for each head: $\frac{\Sigma_\ds |\miedge \cup \gtedge|}{\Sigma_\ds|\miedge|}$.
        %     \item for entire dataset overall: $\Sigma_{head} \frac{\Sigma_\ds |\miedge \cup \gtedge|}{\Sigma_\ds|\miedge|}$.
        % \end{itemize}
    \end{itemize}
    \item Attention analysis draft 2  (node-wise):
    \begin{itemize}
        \item Define $\miedge$ as the set of edges with attention score above a threshold $\theta$.
        \item Define $\mi$ as the set of nodes incident to an edge in $\miedge$.
        \item Define $\gt$ as the result of the bug query.
        % \item Define $\gtedge$ as the cross product of $\gt$.
        \item The metric is the portion of $\mi$ which is also in $\gt$.
        Formula for each attention head: $\frac{\Sigma_\ds |\mi \cap \gt|}{\Sigma_\ds|\mi|}$ where $D$ is the entire dataset.
    \end{itemize}
    \item Interaction matrix $\im \in \mathbb{R}^{|V| \times |V|}$:
    \begin{itemize}
        \item Notes from discussion:
        \begin{itemize}
            \item \ben{How do we order $\gt$ at token-level? One plausible ordering is left-to-right and top-to-bottom. Use line-level for simplicity.}
            \item \ben{How do we order $\gt$?
            \begin{itemize}
                \item Top to bottom (or reverse)
                \item Along the trace order (or reverse)
            \end{itemize}}
            \item \ben{How do we handle truncation? (where at least 1 node is truncated)
            \begin{itemize}
                \item Skip only the truncated edges
                \item Skip the whole example if one edge is truncated
            \end{itemize}}
            \item \ben{How to handle D2A paths?
            \begin{itemize}
                \item Multiple warnings on one function? Analyze each warning separately.
                \item Multiple paths through a function on one warning? Check it out - this may be uncommon or not happen at all.
            \end{itemize}}
            \item \ben{This approach is only defined for multi-step paths.}
            \item \ben{Compute both forward and backward.}
            \item \ben{Baseline: randomly select $|\gt|$ nodes/lines from the function as a path. Order top to bottom.}
            \item \ben{Add a diagram showing the operation of the 2 algorithms on examples.}
        \end{itemize}
        \item Definitions: each cell of $\im$ assigns a probability $\im(v_i, v_j)$ to each pair in $V \times V$ which represents the probability that the node in position $j$ will be attended by the model soon after the node in position $i$.
        $\im(v_i)$ gives the row of probabilities from $i$ to all other positions.
        \item Metric 1: joint probability of $\gt$ according to interaction matrix
        \begin{itemize}
            \item Define $\gtpath = [(\g_1, \g_2), (\g_2, \g_3), \ldots, (\g_{n-1}, \g_{n})]$ where $n = |\gt|$. It has $|\gtpath| = n-1$. \ben{Is it true that $\gtpath \subseteq \gtedge$?}
            % \item given buggy path $bp = [(v_1, v_2), (v_2, v_3), \ldots, (v_{n-1}, v_{n})]$ where $v_i \in V$ and indices correspond to $\gt$ rather than entire set $V$,
            % \item Denote element $i$ of $bp$ as $bp_i = (g_i, g_i+1)$.
            % \item Measure probability of buggy path as $P_{\im}(\gt) = P(bp)$.
            \item By abuse of notation, we want to compute joint probability of the buggy path, denoted $\im(\gtpath)$.
            \item Decompose joint probability $\im(\gtpath)$ into product of probability of each edge $\prod_i^{n-1} \im((\g_i, \g_{i+1}))$. This is possible because, according to the interaction matrix, each edge's probability is independent of the previously traversed path.
            \item Measure probability of buggy path as $P_{\im}(\gtpath) = \prod_i^{n-1} \im((\g_i, \g_{i+1}))$.
            \item Baseline: define $B_{baseline}$ using randomly selected nodes of the same length as $B$.
            \item Presentation: bar chart. X axis = length of path, Y axis = probability.
        \end{itemize}

        \item Metric 2: alignment between induced graph and $\gt$.
        
        % \discussion{\begin{itemize}
        %     \item Consider backwards traversal of buggy path.
        %     \item Consider using threshold instead of selecting top-k; include all interactions where $probability > xxx$.
        % \end{itemize}}
        
        \begin{itemize}
            % \item The interaction matrix is a matrix of real numbers $S \in \mathbb{R}^{m \times m}$ where $m$ is the number of code tokens and each row $S_i$ is a vector of probabilities $[S_{i,1}, \ldots, S_{i,m}]$ where $S_{i,j}$ is the probability of attention moving from token $i$ to token $j$.
            \item $argmax_t(x)$ returns the top-$t$ highest values in a set $x$.
        \end{itemize}
        We propose two ways to compute it.
        Both methods compute a set of nodes which is induced by combining the interaction matrix $\im$ with the bug query $\gt$.
        \begin{itemize}
            \item Algorithm \ref{induction-algorithm-1} builds the longest possible chain out of the top-$t$ most likely connections and computes how what portion of $\gtpath$ was hit. The alignment metric is the length of the induced path.
            \item Algorithm \ref{induction-algorithm-2} builds a (possibly disconnected) graph out of the top-$t$ most likely edges going out of the nodes in $\gtpath$. %and considers fewer disconnected subgraphs to indicate that $\im$ aligns with $\gtpath$.
            The alignment metric is the number of components; fewer is better.
        \end{itemize}

        \input{partials/induction-algorithm-1-longest-possible-chain}
        \input{partials/induction-algorithm-2-most-connected-graph}
        
    \end{itemize}
\end{enumerate}

==> partials/drafts/metrics-01.tex <==
\subsection{Using attention analysis}
\subsubsection{Approach}

\begin{itemize}
    \item a corpus of code sequences $C$ where each example is a sequence of tokens $c_i = [w_1, \ldots, w_m]$,
    \item attention matrix $\alpha \in \mathbb{R}^{m \times m}$,
    \item indicator function $f(w_i, w_j)$ which returns 1 if $w_i$ and $w_j$ are both in $bp$ and 0 otherwise, and
    \item attention threshold $\theta$.
\end{itemize}

Bugs often require multiple operations in order to manifest.
For example, for a buffer overflow to occur, a buffer must be allocated to a certain size, then accessed outside the allocated memory region \citeme{}.
A model that detects the bug precisely in all cases must detect both events.
Conversely, a model that does not detect these events will not be able to detect the bug using its root causes, instead relying on a spurious signal which may often, but will not always, occur with the bug.
To detect the example of a buffer overflow, the model must \textit{attend} to both the allocation (which determines the buffer's size) and the access location (which determines the index at which the buffer is accessed).
\note{Difference from IoU score? Lean into the "multiple events must happen to manifest bug" angle.}

\ben{
Following \cite{wanWhatTheyCapture2022,vigBERTologyMeetsBiology2021}, we analyzed the self-attention scores between tokens in relation to the ground-truth semantics $G$.
\note{Does interaction matrix have any hyperparameters which affect the results?}
Intuitively, a high attention score from token $i$ to token $j$ causes the model to focus more on the previous layer's encoding of token $j$ as it encodes token $i$ \cite{alammar2018illustrated}.
% If the model frequently has a high attention score between the tokens of two statements in $G$, e.g. the buffer allocation location and the buffer overflow location, then it has learned to associate these statements when detecting the bug.
If the model has a high attention score between two statements in $G$, then it has learned that these two statements are important in relation to each other.
This is evidence that the model has learned the semantics of this bug.
% Therefore, we measured how frequently the high attention weights align with $G$ using Formula \ref{formula:attention-analysis}.
Precisely, we compute Equation \ref{formula:attention-analysis}.
}

\begin{equation}\label{formula:attention-analysis}
    p_{\alpha}(f) = \frac
{\sum_{c \in C} \sum_{i = 1}^{|c|} \sum_{j = 1}^{|c|} \mathbbm{1}_{\alpha_{i,j}(c)>\theta} \cdot f(w_i, w_j)}
{\sum_{c \in C} \sum_{i = 1}^{|c|} \sum_{j = 1}^{|c|} \mathbbm{1}_{\alpha_{i,j}(c)>\theta}}
\end{equation}

% Intuitively, we measure, only for the tokens which are above a threshold $\theta$, what proportion are also inside the buggy path.
% If $\mathbbm{1}_{\alpha_{i,j}(c)>\theta}$ is 1 for many tokens in $bp$, then $p_{\alpha}(f)$ will be close to 1.
        
\ben{
Informally, this formula measures the proportion of high-attention pairs (denoted by $1_{\alpha(i,j)}$ which are both present in $G$ (denoted by $f(i,j)$).
\note{Skip f(i,j) generic definition and check whether $i, j \in G$}.
\note Unify notation among all approaches.
}

\subsubsection{Results}

\subsection{Using interaction matrix}
\subsubsection{Approach}

% \ben{This is also the process followed by many static analysis algorithms, albeit automatic.}

% \ben{
% MOTIVATION 1: When a developer debugs, they may follow a thought process, or chain of reasoning, which reproduces the buggy path \citeme{}.
% For example, when debugging a null-pointer dereference bug for a pointer variable $x$, the developer may first note the locations in which $x$ may be assigned NULL, then the locations where $x$ may be dereferenced while its value is still NULL.
% \note{This is similar to the process followed by many static analysis algorithms, albeit automatic.}
% \note Developer debugging process is not really verifiable without a user study, so may not be good motivation.
% }

\ben{
MOTIVATION 2: Many bug semantics are expressed in terms of a sequence of events \citeme{}.
For example, a null pointer dereference manifests when a pointer is assigned to NULL, then may be manipulated, then is dereferenced \citeme{}.
Each event in the sequence is necessary in order to detect the bug, and the events must happen in a certain order (e.g. dereference after assignment to NULL) for the bug to occur.
Vulnerability detection models may detect bugs by \textit{reasoning through} this chain of events.
}

\ben{
Following \cite{paltenghiExtractingMeaningfulAttention2022}, we compared the interaction matrix with ground-truth semantics $G$.
\note{Does interaction matrix have any hyperparameters which affect the results?}
The \textit{interaction matrix} $I$ measures, given a token in the text, which other token of the text will likely be \textit{attended} soon after the current token by the model.
% The interaction graph indicates the probability of attention ``moving'' from one code entity to the next.
Specifically, if the value in the cell $I_{i,j}$ is larger, then the model's attention will likely \textit{move} from token $i$ to token $j$.
\note{define in terms from original paper}
\note{Why is interaction graph necessary apart from attn analysis?}
We repurposed this analysis method in order to understand the model's ``thought process'' when predicting on an example.
Precisely, we compute Equation \ref{formula:interaction-graph} to get the interaction matrix. \note{We extended the definition to bidirectional models since BERT architecture attends to both future and past tokens, unlike GPT-like (decoder-only) models.}
}

\ben{
We developed two metrics which indicate the likelihood of the buggy path given an interaction matrix $I$.
}

\ben{
The first metric measures the joint probability of the entire path as estimated by $I$.
We calculated it using Equation \ref{formula:joint-probability}.
}

\ben{
The second metric measures the joint probability of the entire path as estimated by $I$.
We calculated it using Algorithm \ref{formula:graph-matching}.
It has a hyperparameter $k$, the graph degree.
}

\subsubsection{Results}


\subsection{Using interpretability tools}
\subsubsection{Approach}

\ben{
MOTIVATION: certain statements must be considered important for the prediction in order to detect a bug reliably \citeme{}.
For example, a buffer overflow detector which does not consider the buffer access location cannot definitively answer whether a buffer overflow may occur; it may detect based on heuristics or spurious signals, but will always have additional uncertainty just from ignoring the fault location.
}

\ben{
% We also developed an approach to understand the alignment between $M_{Interpret}$ highlighted by interpretability tools and $G$.
We compared the results of interpretability tools with the ground-truth semantics $G$.
\begin{itemize}
    \item We chose several interpretability tools which have reported useful interpretations \citeme{}.
    \item We aggregated lines using max/mean.
    \item We chose the top-$k$ lines ranked by importance.
    \item We used the IoU metric to measure the alignment.
\end{itemize}
}

\subsubsection{Results}

==> partials/induction-algorithm-1-longest-possible-chain.tex <==
\begin{algorithm}[htbp]
\caption{Induction algorithm 1: longest induced path.}\label{induction-algorithm-1}
\begin{algorithmic}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\newcommand{\Break}{\State \textbf{break}}
\newcommand{\Continue}{\State \textbf{continue}}
\Require $\text{threshold } t = \text{e.g. } 3$
\Require $\text{buggy nodes } \gt = [\g_1, \ldots, \g_n]$
\Require $\text{buggy path } \gtpath = [(\g_1, \g_2), \ldots, (\g_{n-1}, \g_{n})]$
\Require $\text{interaction matrix } \im \in \mathbb{R}^{|V| \times |V|}$
% \Ensure{Longest possible path $M$, induced by $\im$ and $\gt$}
% \Ensure{Length of the longest path induced by $\im$ and $\gt$, edge coverage of $\gt$ induced by $\im$}
\Ensure{(Longest path, edge coverage) of $\gt$ induced by $\im$}

\newcommand{\impath}{currentPath}

% \State $\gtpath = [(\g_1, \g_2), \ldots, (\g_{n-1}, \g_{n})]$

\State $longestPath \gets 0$ \Comment{Length of longest path}
\State $pathLength \gets 0$ \Comment{Length of current path}
\State $edgesCovered \gets 0$ \Comment{\# of edges covered by $\im$ in $\gtpath$}
% \State $head \gets \g_1$ \Comment{Current head of $\impath$}
% \State $\impath \gets [head]$ \Comment{Path induced by interaction matrix}
\For{$i \in [1 \ldots |\gtpath|]$} %\Comment{\ben{todo add reverse direction}}
    \State $mostLikely = argmax_t\{\im(\g_i)\}$
    \If{$\g_{i+1} \in mostLikely$} \Comment{Add to current path}
        % \State $head \gets \g_{i}$
        % \State $\impath.append(head)$
        \State $pathLength \gets pathLength + 1$
        \State $edgesCovered \gets edgesCovered + 1$
        \If{$longestPath < pathLength$}
            \State $longestPath \gets pathLength$
        \EndIf
    \Else \Comment{End the current path and start a new path}
        \State $pathLength \gets 0$
    \EndIf
\EndFor
% \If{$longestPath < pathLength$}
%     \State $longestPath \gets pathLength$
% \EndIf

% \State $M \gets longest(paths)$
% \State $numEdges \gets |\gtpath|$

% \State \Return $\frac{|\gtpath \cap \impath|}{|\gtpath|}$
% \State \Return $\frac{|M|}{|\gtpath|}$ \Comment{$\im \approx \gtpath \Leftrightarrow$ longer path}


\State \Return $\frac{longestPath}{|\gtpath|}$,
$\frac{edgesCovered}{|\gtpath|}$
% \Comment{$\im \approx \gtpath \Leftrightarrow$ longer path}

\end{algorithmic}
\end{algorithm}


==> partials/induction-algorithm-2-most-connected-graph.tex <==
\begin{algorithm}[htbp]
\caption{Induction algorithm 2: most connected graph. \ben{Complicated - improve it. Consider inducing graph with only $\im$, not $\gt$, using threshold probability, then compare with $\gt$. Node/edge coverage are not as interesting as paths because they're covered by attention and interpretability analysis.}}\label{induction-algorithm-2}
\begin{algorithmic}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\Require $\text{threshold } t = \text{e.g. } 3$
\Require $\text{buggy path } \gt = [\g_1, \ldots, \g_n]$
\Require $\text{interaction matrix } \im \in \mathbb{R}^{|V| \times |V|}$
% \Ensure{Nodes of graph $M$, induced by $\im$ and $\gt$}
\Ensure{Number of components in the graph induced by $\im$ and $\gt$}

\newcommand{\imgraph}{M}

\State $\imgraph \gets$ empty graph
\For{$i \in [1 \ldots n]$}
    \State \Comment{\parbox[t]{0.9\linewidth}{If $\g_i \in V[\imgraph]$, then this line will extend the existing graph. Otherwise, it will begin a disconnected subgraph.}} % https://tex.stackexchange.com/a/63667
    \State $V[\imgraph] \gets V[\imgraph] \cup \g_i$
    \State $mostLikely = argmax_t\{\im(\g_i)\}$
    \For{$j \in [1 \ldots t]$} \Comment{Connect $b_i$ to succeeding nodes}
        \State $E \gets E \cup (\g_i, mostLikely_j)$
    \EndFor
\EndFor

% \State \Return $V[\imgraph]$
\State \Return $|components(\imgraph)|$ \Comment{\parbox[t]{.4\linewidth}{$\im \approx \gtpath \Leftrightarrow$ few disconnected subgraphs}}

\end{algorithmic}
\end{algorithm}


==> partials/reproduced-performance-acc-f1-mixed.tex <==
\begin{table}[htbp]
    \centering
    % \rowcolors{2}{gray!5}{white}
    \caption{Reproduced model performance \ben{Acc/F1 mixed}}
    \label{tab:reproduced-performance}
    \begin{tabular}{l|c|c|c|c}
        \hline
        % \rowcolor{gray!15}
        {\bf Model} & \makecell{{\bf D2A}\\Accuracy} & \makecell{{\bf Devign}\\Accuracy} & \makecell{{\bf Big-Vul}\\F1} & \makecell{{\bf ReVeal}\\F1} \\\hline
CodeBERT      & 61.91 & 64.57 & 40.65 & 64.11 \\ \hline
GraphCodeBERT & 61.74 & 62.59 & 38.55 & 60.50 \\ \hline
UniXcoder     & 60.57 & 63.65 & 39.55 & 62.88 \\ \hline
CodeT5        & 55.54 & 64.82 & 40.20 & 62.71 \\ \hline
LineVul       & 58.72 & 62.30 & 86.04 & 59.09 \\ \hline
% numbers for full D2A data
% Model	D2A
% CodeBERT	63.93
% GraphCodeBERT	61.65
% UniXcoder	61.81
% CodeT5	60.36
% LineVul	61.65
% Updated numbers for restricted D2A data
% Model	D2A
% CodeBERT	61.91
% GraphCodeBERT	61.74
% UniXcoder	60.57
% CodeT5	55.54
% LineVul	58.72
% VulBERTa &  &  &  &  \\ \hline
    \end{tabular}
\end{table}
